Gradual Typing for Extensibility by Rows

This work studies gradual typing for row types and row polymorphism. Key ingredients in this work are the dynamic row type, which represents a statically unknown part of a row, and consistency for row types, which allows injecting static row types into the dynamic row type and, conversely, projecting the dynamic row type to any static row type. While consistency captures the behavior of the dynamic row type statically, it makes the semantics of a gradually typed language incoherent when combined with row equivalence which identifies row types up to field reordering. To solve this problem, we develop consistent equivalence, which characterizes composition of consistency and row equivalence. Using consistent equivalence, we propose a polymorphic blame calculus for row types and row polymorphism. In our blame calculus, casts perform not only run-time checking with the dynamic row type but also field reordering in row types. To simplify our technical development for row polymorphism, we adopt scoped labels, which are employed by the language Koka and are also emerging in the context of effect systems. We give the formal definition of our blame calculus with these technical developments and prove its type soundness. We also sketch the gradually typed surface language and type-preserving translation from the surface language to the blame calculus and discuss conservativity of the surface language over typing of a statically typed language with row types and row polymorphism.

==> defns/grad_lang/typing_rules.tex <==
\ifthen{\boolean{show-common}}{
$\ottdruleTgXXVar{}$ \hfil
$\ottdruleTgXXConst{}$ \hfil
$\ottdruleTgXXLam{}$ \\[3ex]
$\ottdruleTgXXApp{}$ \\[3ex]
$\ottdruleTgXXTLam{}$ \hfil
$\ottdruleTgXXTApp{}$ \\[3ex]
$\ottdruleTgXXREmp{}$ \hfil
$\ottdruleTgXXRExt{}$ \\[3ex]
$\ottdruleTgXXRLet{}$ \\[3ex]
}
\ifthen{\boolean{show-variant}}{
$\ottdruleTgXXVInj{}$ \hfil
$\ottdruleTgXXVLift{}$ \\[3ex]
$\ottdruleTgXXVCase{}$ \hfil
}


==> defns/static_lang.eval.tex <==
\textbf{Evaluation rule} \quad \framebox{$ \ottnt{M_{{\mathrm{1}}}}  \mathrel{ \makestatic{\longrightarrow} }  \ottnt{M_{{\mathrm{2}}}} $}
%
\begin{center}
 $\ottdruleEsXXRed{}$
\end{center}


==> defns/static_lang.reduction.tex <==
\textbf{Reduction rules} \quad \framebox{$ \ottnt{M_{{\mathrm{1}}}}  \mathrel{ \makestatic{\rightsquigarrow} }  \ottnt{M_{{\mathrm{2}}}} $}
%
\[\begin{array}{rclll}
 % beta reduction
 \kappa_{{\mathrm{1}}} \, \kappa_{{\mathrm{2}}} &  \makestatic{\rightsquigarrow} 
 &  \zeta  (  \kappa_{{\mathrm{1}}}  ,  \kappa_{{\mathrm{2}}}  ) 
 && \Rs{Const} \\
 %
 \ottsym{(}   \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \ottnt{M}  \ottsym{)} \, w &  \makestatic{\rightsquigarrow} 
 & \ottnt{M} \,  [  w  \ottsym{/}  \mathit{x}  ] 
 && \Rs{Beta} \\
 %
 \ottsym{(}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M}  \ottsym{)} \, \ottnt{A} &  \makestatic{\rightsquigarrow} 
 & \ottnt{M} \,  [  \ottnt{A}  /  \mathit{X}  ] 
 && \Rs{TyBeta} \\
 %
 \mathsf{let} \, \ottsym{\{}  \ell  \ottsym{=}  \mathit{x}  \ottsym{;}  \mathit{y}  \ottsym{\}}  \ottsym{=}  w \, \mathsf{in} \, \ottnt{M_{{\mathrm{2}}}} &  \makestatic{\rightsquigarrow} 
 & \ottnt{M} \,  [  w_{{\mathrm{1}}}  \ottsym{/}  \mathit{x}  \ottsym{,}  w_{{\mathrm{2}}}  \ottsym{/}  \mathit{y}  ]  & \text{(if $w \,  \triangleright _{ \ell }  \, w_{{\mathrm{1}}}  \ottsym{,}  w_{{\mathrm{2}}}$)}
 & \Rs{Record} \\
 %
  \variantlift{ \ell }{ \ottnt{A} }{ \ottsym{(}   { w }^{ \ell' }   \ottsym{)} }  &  \makestatic{\rightsquigarrow} 
 &  { w }^{ \ell' }  & \text{(if $\ell \,  \not=  \, \ell'$)}
 & \Rs{Embed} \\
 %
  \mathsf{case} \,  \ottsym{(}  \ell \, w  \ottsym{)}  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle  &  \makestatic{\rightsquigarrow} 
 & \ottnt{M_{{\mathrm{1}}}} \,  [  w  \ottsym{/}  \mathit{x}  ] 
 && \Rs{CaseL} \\
 %
  \mathsf{case} \,   \variantlift{ \ell }{ \ottnt{A} }{ \ottsym{(}   { w }^{ \ell }   \ottsym{)} }   \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle  &  \makestatic{\rightsquigarrow} 
 & \ottnt{M_{{\mathrm{2}}}} \,  [   { w }^{ \ell }   \ottsym{/}  \mathit{x}  ] 
 && \Rs{CaseR1} \\
 % \texttt{\textcolor{red}{<<no parses (char 25): case lift<l:A> (lift<l:<B***>> (l w)) with l x -> M1; y -> M2 >>}} &  \makestatic{\rightsquigarrow}  & \texttt{\textcolor{red}{<<no parses (char 12): M2\{lift<l:<B***>> (l w)/x\} >>}} & \Rs{CaseR1} \\
 %
  \mathsf{case} \,   { w }^{ \ell' }   \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle  &  \makestatic{\rightsquigarrow} 
 & \ottnt{M_{{\mathrm{2}}}} \,  [   { w }^{ \ell' }   \ottsym{/}  \mathit{x}  ]  & \text{(if $\ell \,  \not=  \, \ell'$)}
 & \Rs{CaseR2} \\
 % \texttt{\textcolor{red}{<<no parses (char 15): case lift<l':<A***>> (l' w) with l x -> M1; y -> M2 >>}} &  \makestatic{\rightsquigarrow}  & \texttt{\textcolor{red}{<<no parses (char 13): M2\{lift<l':<A***>> (l' w)/x\} >>}} & \Rs{CaseR2} \\
 %
  \end{array}\]


==> defns/static_lang.syntax.tex <==
\[
\begin{array}{lrl}
 \multicolumn{3}{l}{
  \textbf{Variables for types and rows} \quad \mathit{X}
  \qquad
  \textbf{Kinds} \quad \ottnt{K} ::=  \mathsf{T}  \mid  \mathsf{R} 
  } \\[1ex]

 \textbf{Base types} \hfill
  \iota  & ::= &  \mathsf{bool}  \mid  \mathsf{int}  \mid ... \\[.5ex]

 \textbf{Types and rows} \quad \hfill
  \ottnt{A}, \ottnt{B}, \ottnt{C}, \ottnt{D}, \rho & ::= &
                      \mathit{X} \mid
                      \iota \mid \ottnt{A}  \rightarrow  \ottnt{B} \mid  \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{A} \mid
                       [  \rho  ]  \mid  \langle  \rho  \rangle  \mid
                      % rows
                       \cdot  \mid   \ell  \mathbin{:}  \ottnt{A}   ;  \rho 
                      \\[.5ex]

 \textbf{Constants} \hfill
  \kappa & ::= &  \mathsf{true}  \mid  \mathsf{false}  \mid \ottsym{0} \mid  \mathsf{+}  \mid ... \\[.5ex]

 \textbf{Terms} \hfill
  \ottnt{M}   & ::= & \mathit{x} \mid \kappa \mid  \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \ottnt{M} \mid \ottnt{M_{{\mathrm{1}}}} \, \ottnt{M_{{\mathrm{2}}}} \mid
                   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M} \mid \ottnt{M} \, \ottnt{A} \mid \\ &&
                  \ottsym{\{}  \ottsym{\}} \mid \ottsym{\{}  \ell  \ottsym{=}  \ottnt{M_{{\mathrm{1}}}}  \ottsym{;}  \ottnt{M_{{\mathrm{2}}}}  \ottsym{\}} \mid
                  \mathsf{let} \, \ottsym{\{}  \ell  \ottsym{=}  \mathit{x}  \ottsym{;}  \mathit{y}  \ottsym{\}}  \ottsym{=}  \ottnt{M_{{\mathrm{1}}}} \, \mathsf{in} \, \ottnt{M_{{\mathrm{2}}}} \mid \\ &&
                  \ell \, \ottnt{M} \mid  \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} }  \mid
                   \mathsf{case} \,  \ottnt{M}  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle 
                  \\[.5ex]

 \textbf{Values} \hfill
  w        & ::= & \kappa \mid  \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \ottnt{M} \mid  \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M} \mid
                       \ottsym{\{}  \ottsym{\}} \mid \ottsym{\{}  \ell  \ottsym{=}  w_{{\mathrm{1}}}  \ottsym{;}  w_{{\mathrm{2}}}  \ottsym{\}} \mid
                        { w }^{ \ell } 
                       \\ \hfill
  { w }^{ \ell }  & ::= & \ell \, w \mid  \variantlift{ \ell }{ \ottnt{A} }{  { w }^{ \ell }  } 
                       \\[1ex]

 \textbf{Evaluation contexts} \hfill
  F & ::= &  [\,]  \mid F \, \ottnt{M_{{\mathrm{2}}}} \mid w_{{\mathrm{1}}} \, F \mid F \, \ottnt{A} \mid
                \ottsym{\{}  \ell  \ottsym{=}  F  \ottsym{;}  \ottnt{M_{{\mathrm{2}}}}  \ottsym{\}} \mid \ottsym{\{}  \ell  \ottsym{=}  w_{{\mathrm{1}}}  \ottsym{;}  F  \ottsym{\}} \mid \\ &&
                \mathsf{let} \, \ottsym{\{}  \ell  \ottsym{=}  \mathit{x}  \ottsym{;}  \mathit{y}  \ottsym{\}}  \ottsym{=}  F \, \mathsf{in} \, \ottnt{M_{{\mathrm{2}}}} \mid \\ &&
                \ell \, F \mid  \variantlift{ \ell }{ \ottnt{A} }{ F }  \mid
                 \mathsf{case} \,  F  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle 
                \\[.5ex]

 \textbf{Typing contexts} \hfill
  \Gamma   & ::= &  \emptyset  \mid \Gamma  \ottsym{,}   \mathit{x}  \mathord{:}  \ottnt{A}  \mid \Gamma  \ottsym{,}   \mathit{X}  \mathord{:}  \ottnt{K}  \\[.5ex]
\end{array}\]


==> defns/static_lang.typing.tex <==
\textbf{Typing rules} \quad
\framebox{$ \Gamma  \mathrel{ \makestatic{\vdash} }  \ottnt{M}  :  \ottnt{A} $}
%
\begin{center}
 $\ottdruleTsXXVar{}$ \hfil
 $\ottdruleTsXXConst{}$ \hfil
 $\ottdruleTsXXLam{}$ \\[3ex]
 $\ottdruleTsXXApp{}$ \hfil
 $\ottdruleTsXXTLam{}$ \\[3ex]
 $\ottdruleTsXXTApp{}$ \hfil
 $\ottdruleTsXXREmp{}$ \\[3ex]
 $\ottdruleTsXXRExt{}$ \hfil
 $\ottdruleTsXXRLet{}$ \\[3ex]
 $\ottdruleTsXXVInj{}$ \hfil
 $\ottdruleTsXXVLift{}$ \\[3ex]
 $\ottdruleTsXXVCase{}$ \\[3ex]
 $\ottdruleTsXXEquiv{}$
\end{center}


==> defns/static_lang.wf.tex <==
\textbf{Well-formedness rules for typing contexts, types, and rows} \\[1ex]
\framebox{$ \mathrel{ \makestatic{\vdash} }  \Gamma $} \quad
%
\begin{center}
 $\ottdruleWFsXXEmpty{}$ \hfil
 $\ottdruleWFsXXExtVar{}$ \\[3ex]
 $\ottdruleWFsXXExtTyVar{}$
\end{center}

\framebox{$ \makestatic{\Gamma}  \mathrel{ \makestatic{\vdash} }  \makestatic{\mathit{A} }  :  \ottnt{K} $} \quad
\begin{center}
 $\ottdruleWFsXXTyVar{}$ \hfil
 $\ottdruleWFsXXDyn{}$ \hfil
 $\ottdruleWFsXXBase{}$ \\[3ex]
 $\ottdruleWFsXXFun{}$ \hfil
 $\ottdruleWFsXXPoly{}$ \hfil
 $\ottdruleWFsXXRecord{}$ \\[3ex]
 $\ottdruleWFsXXVariant{}$ \hfil
 $\ottdruleWFsXXREmp{}$ \hfil
 $\ottdruleWFsXXCons{}$
\end{center}


==> defns/static_lang/eval1.tex <==
\textbf{Evaluation rule} \quad \framebox{$ \ottnt{M_{{\mathrm{1}}}}  \mathrel{ \makestatic{\longrightarrow} }  \ottnt{M_{{\mathrm{2}}}} $}
%
\[
   F  [  \ottnt{M_{{\mathrm{1}}}}  ]   \mathrel{ \makestatic{\longrightarrow} }   F  [  \ottnt{M_{{\mathrm{2}}}}  ]   \quad \text{(if $ \ottnt{M_{{\mathrm{1}}}}  \mathrel{ \makestatic{\rightsquigarrow} }  \ottnt{M_{{\mathrm{2}}}} $)} \qquad \EsWoP{Red}
\]
\begin{center}
 $\ottdruleEsXXRed{}$
\end{center}


==> sections/_grad_lang.tex <==
\setboolean{show-common}{true}
\setboolean{shade-common}{true}
\setboolean{show-variant}{false}
\setboolean{show-grad}{true}
\setboolean{show-grad-term}{true}
\setboolean{show-typename}{false}
\setbool{shade-dyn}{false}

\section{{\surfacelang}: A gradually typed counterpart of {\staticlang}}

\begin{figure}[t]
 \input{defns/grad_lang/syntax}
 \caption{Syntax of {\surfacelang}.}
 \label{fig:grad_lang:syntax}
\end{figure}

This section presents our language {\surfacelang}, a gradually typed counterpart
of {\staticlang} given in \sect{static_lang}.
%
% We will extend {\staticlang} and
% its counterpart with variant types in \sect{ext} after seeing how row types with
% scoped labels and row polymorphism can be handled in gradual typing through this
% and the next sections.
%
The syntax of {\surfacelang} is almost the same as that of {\staticlang}; see
\reffig{grad_lang:syntax}, where the parts shared with {\staticlang} are displayed in gray.
The only difference is the addition of the dynamic type $ \star $ for value types
and row types.  The dynamic row type is just the dynamic type used in a position
requiring row types.

In the rest of this section, we present the type system of {\surfacelang}; the
semantics will be given via translation to a polymorphic blame calculus
{\interlang} in \sect{...}.  The key ingredient of the type system is
\emph{consistency}.  Consistency of {\surfacelang} is influenced by not only the
dynamic row type but also field reordering.  We first formalize consistency and
then introduce \emph{consistent equivalence} to resolve common issues of
consistency combined with subsumption like
subtyping~\cite{Siek/Taha_2007_ECOOP} \AI{What is ``subsumption like subtyping''?}.  Once we develop consistency and
consistent equivalence, the type system of {\surfacelang} is derived naturally
from that of {\staticlang}.

\subsection{Consistency}

Consistency $ \sim $ is a fundamental block of a static aspect of gradual typing
and decides possible interaction between statically typed and dynamically typed
code.  Usually, it is defined as a binary relation between types and,
intuitively, types are consistent if casts between them could
be successful.  For example, statically typed values can be injected to the
dynamic type and, conversely, dynamically typed values could be projected to any
type (whether a cast succeeds depends on whether run-time values can
behave as the target type of the cast, though).  This idea is axiomatized by the
following two rules.
\[
 \ottnt{A}  \sim  \star \qquad \star  \sim  \ottnt{A}
\]
Consistency is also defined so that type constructors are compatible with it.
For example, a consistency rule for function types is:
\[
 \frac{\ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad \ottnt{B_{{\mathrm{1}}}}  \sim  \ottnt{B_{{\mathrm{2}}}}}{\ottnt{A_{{\mathrm{1}}}}  \rightarrow  \ottnt{A_{{\mathrm{2}}}}  \sim  \ottnt{B_{{\mathrm{1}}}}  \rightarrow  \ottnt{B_{{\mathrm{2}}}}}
\]

In what follows, we discuss how to extend consistency to deal with row types and
universal types and then give its formal definition.  While that definition is
reasonable, it causes issues on typechecking and semantics.  These issues
motivate us to introduce consistent equivalence.

\subsubsection{Consistency for row types}
%
A trivial extension of consistency to row types is to allow relating the dynamic
row type to any row type ($\rho  \sim  \star$ and $\star  \sim  \rho$) and to add the
following compatible rule for row extension.
\[
  \frac{\ottnt{A}  \sim  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim    \ell  \mathbin{:}  \ottnt{B}   ;  \rho_{{\mathrm{2}}} }
\]
This rule makes, e.g., $\ottsym{(}    \ell  \mathbin{:}   \mathsf{int}    ;   \cdot    \ottsym{)}$ and $\ottsym{(}    \ell  \mathbin{:}  \star   ;   \cdot    \ottsym{)}$ consistent.

While necessary and reasonable, this compatibility rule is not sufficient to
contain all pairs of row types such that casts between them could
be successful.  The problem is in a case that row types to be related end with
$ \star $ (i.e., they take the form $  \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A_{{\mathrm{1}}}}   ;  ...  ;    \ell_{\ottmv{n}}  \mathbin{:}  \ottnt{A_{\ottmv{n}}}   ;  \star  $)
and they hold field labels distinct from those of each other.  For example, let
us consider row types $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.  While these row types are not consistent only with the above extension
of consistency, it is desirable that they are consistent because casts
between record types and between variant types with these row types could be
successful: casts between record types $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   ] $ and
$ [    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   ] $ could be successful because a record value of either of
<<<<<<< HEAD
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields \AI{Remove ``fields''?}; similarly, type conversion
=======
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields; similarly, casts
>>>>>>> master
between variant types $ \langle    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \rangle $ and $ \langle    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \rangle $
could be successful because they accommodate both of values injected with
$\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$.  It is notable that the assumption that $\ell_{{\mathrm{1}}}$ and
$\ell_{{\mathrm{2}}}$ are different labels is critical here;
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;  \star $ should not be consistent since the
types $ \mathsf{int} $ and $ \mathsf{str} $ of their $\ell$ fields are inconsistent.
\AI{More elaboration? $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;   \cdot     ] $. }

The example showing insufficiency of the simple extension above gives a
guideline to design a new consistency rule for row extension: given consistent
row types $\rho_{{\mathrm{1}}}$ and $\rho_{{\mathrm{2}}}$, extension of $\rho_{{\mathrm{1}}}$ with label $\ell$
preserves consistency with $\rho_{{\mathrm{2}}}$ if $\rho_{{\mathrm{2}}}$ ends with $ \star $ and $\ell$
does not appear in $\rho_{{\mathrm{2}}}$ .  Formally:
\[
 \frac{\quad  \rho_{{\mathrm{2}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim  \rho_{{\mathrm{2}}}}
\]
where $\mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)}$ is the set of the field labels of $\rho_{{\mathrm{2}}}$.  This rule is
justified by the intuition that: first, the occurrence of $ \star $ in $\rho_{{\mathrm{2}}}$
allows assuming that $\rho_{{\mathrm{2}}}$ could contain a field of $ \ell  \mathbin{:}  \star $; and
then the $\ell$ field can move to the head of $\rho_{{\mathrm{2}}}$ by type-and-row
equivalence since $\rho_{{\mathrm{2}}}$ is assumed not to have other $\ell$ fields.
We can apply the same discussion for extension of $\rho_{{\mathrm{2}}}$:
\[
 \frac{\quad  \rho_{{\mathrm{1}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{1}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{\rho_{{\mathrm{1}}}  \sim    \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{2}}} }
\]
Use of these two rules make row types $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \ottsym{)}$ consistent.


\subsubsection{Consistency for universal types}
%
Consistency for universal types in this work follows the earlier work on
polymorphic gradual typing by \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}.
Their consistency relates not only a universal type to another one but also a
universal type to what they call a non-$\forall$ type (i.e., a type such that
its top type constructor is not $\forall$).  The flexibility of their
consistency enables interaction between statically typed code with polymorphism
and dynamically typed code without polymorphism.  For example, in their work,
universal type $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ is consistent with non-$\forall$ type
$\star  \rightarrow  \star$.  Igarashi et al.\ present a few conditions on non-$\forall$
types to be consistent with universal types; non-$\forall$ types satisfying the
conditions are called \emph{quasi}-universal types\footnote{{Igarashi et al.}
call such types quasi-polymorphic types, but we use that term for consistent use
of terminology.} because they are not actual universal types but could behave as
them by casts.  We adjust their notion of quasi-universal
types to our setting with row types.
%
\input{defns/grad_lang/quasi-universal}
%
Then, we introduce a consistency rule like:
\[
 \frac{\quad \mathbf{QPoly} \, \ottsym{(}  \ottnt{A_{{\mathrm{2}}}}  \ottsym{)} \quad \mathit{X} \,  \not\in  \,  \mathit{ftv}  (  \ottnt{A_{{\mathrm{2}}}}  )  \quad \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad}{ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}}}
\]
and its symmetric version.

We make a remark on other choices of consistency for universal types.
\citet{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP}
give \emph{compatibility} instead of consistency.  Their compatibility is
designed to capture as many possibly successful casts as
possible, and, as a result, it deems even perhaps apparently incompatible
types---e.g., $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ and $ \mathsf{int}   \rightarrow   \mathsf{str} $---compatible.  In return for
this great flexibility, their calculus lacks conservativity over typing of
System F, the underlying calculus of their gradually typed language (i.e., a
static typing error found by System F may not be found by their gradual type
system).  Another definition of consistency is also given by
\citet{Toro/Labrada/Tanter_2019_POPL}.  Their consistency relates a universal
type only to another universal type and not to any non-$\forall$ type.  Their
gradually typed language achieves conservativity over typing of System F, but
that \AI{the?} strict distinction between universal types and non-$\forall$ types
disallows dynamically typed code, where no type information appears, to use
polymorphic values.  For example, let us consider a program $\ottnt{M} \defeq
 \lambda\!  \,  \mathit{f}  \mathord{:}  \star   \ottsym{.}  \mathit{f} \,  0 $, which calls function $\mathit{f}$ of the dynamic type $ \star $ with
integer $\ottsym{0}$.  In Toro et al.'s language, any application of $\ottnt{M}$ to a
polymorphic function would raise an exception:
\[
 \ottnt{M} \, \ottsym{(}   \Lambda\!  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \,  \lambda\!  \,  \mathit{x}  \mathord{:}  \mathit{X}   \ottsym{.}  \mathit{x}  \ottsym{)}  \longrightarrow^{*}  \mathsf{blame} \, \ottnt{p}
\]
because polymorphic values can be used successfully only if it is applied to
types.  This means that polymorphic values cannot be used in dynamically typed
code because it should have no type information including type application.

We adopt the consistency style of \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}
\AI{``The consistency style'' doesn't make sense.}
because of its balance between flexibility---it allows dynamically typed code to
use polymorphic values---and strictness \AI{I'm not sure ``strict''/''strictness'' is a right word.}---it makes a gradually typed language
conservative over typing of System F.  However, we believe that how to deal with
universal types in consistency is orthogonal to consistency for row types and
that we can choose a suitable treatment depending on a case.
\AI{cases?}


\subsubsection{Formal definition}
%
Now, we present a formal definition of consistency for {\surfacelang}.  We start
with formalizing the notions used in the consistency rules for row extension.
%
\input{defns/grad_lang/labels_in_row}
\input{defns/grad_lang/row_concat}
\input{defns/grad_lang/row_ends_with_dyn}
\AI{Do you have to define ``ending with $ \star $'' in terms of concatenation?
I thought you could define as a simple recursively defined predicate.}

We say that a relation between types is compatible if and only if it is closed
under type and row constructors.

\begin{figure}[t]
 \input{defns/grad_lang/consistency}
 \caption{Consistency.}
 \label{fig:grad_lang:consistency}
\end{figure}

\begin{defn}[Consistency]
 Consistency $\ottnt{A}  \sim  \ottnt{B}$ is the smallest compatible relation satisfying the
 rules given by \reffig{grad_lang:consistency}.
\end{defn}

\subsubsection{Issues of consistency combined with type-and-row equivalence}
\label{sec:consistency-issue}
%
Consistency does not subsume type-and-row equivalence.  Thus, if {\surfacelang}
incorporated consistency directly, it would be used combined with type-and-row
equivalence, especially in the form of composition $ \equiv  \circ  \sim $.
However, use of that composition gives rise to two issues, which were first
found in the work on gradual typing for subtyping~\cite{Siek/Taha_2007_ECOOP}.
The first issue is on typechecking.  If {\surfacelang} incorporated consistency
in the form of the composition, its typechecking algorithm would have to decide
whether given two types $\ottnt{A}$ and $\ottnt{B}$ are contained in the
composition. Thus, it would need to find an intermediate type $\ottnt{C}$ such that
$\ottnt{A}  \equiv  \ottnt{C}$ and $\ottnt{C}  \sim  \ottnt{B}$.  But, how?  This issue may not be as serious as the
case of subtyping~\cite{Siek/Taha_2007_ECOOP} because $ \equiv $ just reorders
fields in a row, but it should be still resolved.  The second issue is
more serious: incoherent semantics.  For example, let us consider the
following term
\[
\ottnt{M} \defeq \ottsym{\{}  \ell_{{\mathrm{1}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}  \ottsym{;}  \ottsym{\{}  \ell_{{\mathrm{2}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}  \ottsym{;}  \ottsym{\{}  \ottsym{\}}  \ottsym{\}}  \ottsym{\}}  \ottsym{:}  \star
\]
where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$, $\ottnt{M_{{\mathrm{1}}}}$ is a divergent term, and $\ottnt{M_{{\mathrm{2}}}}$ is a term
raising an exception (we write $\ottnt{M'}  \ottsym{:}  \ottnt{A}$ for ascription, which is a shorthand
of $\ottsym{(}   \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \mathit{x}  \ottsym{)} \, \ottnt{M'}$).  Similar to the earlier calculi for polymorphic gradual
typing~\cite{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP,Igarashi/Sekiyama/Igarashi_2017_ICFP},
evaluation of this term in {\surfacelang} would trigger application of
$ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ or $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$ to $ \star $.  \AI{Is it so clear that such an application takes place?}  But, which?  If $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ were \AI{Why subjunctive mood?}
applied, the evaluation result would be divergence; otherwise, if $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$
were, the result would be a failure of run-time checking.  Actually, which is
chosen would be determined by intermediate type $\rho$ that proves $ [    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     ]   \equiv   [  \rho  ] $ and $ [  \rho  ]   \sim  \star$ in a typing
derivation for $\ottnt{M}$, because translation of a gradually typed term to a blame
calculus depends on instances of consistency found in the
derivation~\cite{Siek/Taha_2006_SFPW}.  The problem here is that $\rho$ cannot
be determined to be unique: both of $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ can be chosen.  Although we might be able to design
coherent semantics with respect to field reordering, we take an approach more
standard in gradual
typing~\cite{Siek/Taha_2007_ECOOP,Xie/Bi/Oliveira_2018_ESOP}.

\subsection{Consistent equivalence}

To resolve the issues on consistency, we give \emph{consistent equivalence}
$ \simeq $, which characterizes composition of consistency and type-and-row
equivalence.  Our idea is to extend the consistency rules for row
extension---\Cns{ConsL} and \Cns{ConsR}---so that both cases that a label used
for extension on one side does and does not appear in a row on the other side
are taken into account; consistency handles only the latter case.  A promising
rule that handles only the former case is like:
\[
 \frac{\rho_{{\mathrm{2}}}  \equiv    \ell  \mathbin{:}  \ottnt{B}   ;  \rho'_{{\mathrm{2}}}  \quad \ottnt{A}  \simeq  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho'_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}}
\]
We merge this rule and \Cns{ConsL} into a single rule as follows.  First, we
split $\rho_{{\mathrm{2}}}$ into the first field labeled with $\ell$ and the remaining row;
these field and row correspond to $ \ell  \mathbin{:}  \ottnt{B} $ and $\rho'_{{\mathrm{2}}}$ in the rule above,
respectively.  Even in the case that $\rho_{{\mathrm{2}}}$ includes no field labeled with
$\ell$, \emph{if $\rho_{{\mathrm{2}}}$ ends with $ \star $}, then we can \emph{suppose} that
$\rho_{{\mathrm{2}}}$ includes a $\ell$ field because the dynamic row type can be supposed
to be any row type.  Since we have no idea about a type of such a $\ell$ field,
we regard it as the dynamic type conservatively.  Finally, we check consistency
between $\ottnt{A}$ and the type of the $\ell$ field extracted from $\rho_{{\mathrm{2}}}$ and
between $\rho_{{\mathrm{1}}}$ and the remaining row.

\begin{figure}[t]
 \input{defns/grad_lang/consistent_equiv}
 \caption{Consistent equivalence.}
 \label{fig:grad_lang:consistent-equiv}
\end{figure}

The idea above to merge is formalized by the consistent equivalence rule
\CE{ConsL} in \reffig{grad_lang:consistent-equiv}; there \CE{ConsR} is the
symmetric version of \CE{ConsL} and other rules have the same form as the
corresponding rules for consistency.
%
In \CE{ConsL} and \CE{ConsR}, $\rho_{{\mathrm{1}}} \,  \triangleright _{ \ell }  \, \ottnt{A}  \ottsym{,}  \rho_{{\mathrm{2}}}$ is a formalization of the
``split'' operation on row types, defined as follows.
%
\input{defns/grad_lang/row_split}
%
\begin{defn}[Consistent equivalence]
 Consistent equivalence $\ottnt{A}  \simeq  \ottnt{B}$ is the smallest compatible relation
 satisfying the rules given by \reffig{grad_lang:consistent-equiv}.
\end{defn}

We can confirm that consistent equivalence subsumes both consistency and
type-and-row equivalence by examples.  For example,
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \simeq    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ and
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ are derivable if $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.
More generally, it subsumes the composition of consistency and type-and-row
equivalence.  We can show (and actually showed) that $ \simeq $ coincides with
$ \equiv  \circ  \simeq $, but, following \citet{Xie/Bi/Oliveira_2018_ESOP}, we prove
another form of equivalence between $ \simeq $ and combination of $ \equiv $ and
$ \simeq $; the statement in this form expects us to incorporate implicit
higher-order polymorphism easily.
%
\begin{theorem}
 \label{thm:consistent-eq-consistent-equiv}
 $\ottnt{A}  \simeq  \ottnt{B}$ if and only if $\ottnt{A}  \equiv  \ottnt{A'}$ and $\ottnt{A'}  \sim  \ottnt{B'}$ and $\ottnt{B'}  \equiv  \ottnt{B}$
 for some $\ottnt{A'}$ and $\ottnt{B'}$.
\end{theorem}

We will develop the type system of {\surfacelang} using consistent equivalence in
\sect{grad_lang:typing}.  The type system does not rest on consistency, so it
does not cause the issues on typechecking nor semantics raised by consistency.
%
A typechecking algorithm for the type system does not need to infer an
intermediate type because it is enough to check if given two types are in a
single relation, consistent equivalence.  At first glance, one might consider
that it is problematic that some consistent equivalence rules are not
syntax-directed.  For example, when we would like to derive
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$, it may appear unclear which
rule of \CE{ConsL} and \CE{ConsR} should be applied first.  Fortunately, either
is fine, which is shown by the following lemma together with symmetry of
consistent subtyping.
%
\begin{lemma}%{consistent-inv-cons}
 If $  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}$,
 then $\rho_{{\mathrm{2}}} \,  \triangleright _{ \ell }  \, \ottnt{B}  \ottsym{,}  \rho'_{{\mathrm{2}}}$ and $\ottnt{A}  \simeq  \ottnt{B}$ and $\rho_{{\mathrm{1}}}  \simeq  \rho'_{{\mathrm{2}}}$.
\end{lemma}
%
For semantics, use of consistent subtyping makes the typing rules
syntax-directed, and, therefore, derivations for a typing judgment are
determined uniquely.


\subsection{Type system}
\label{sec:grad_lang:typing}

\begin{figure}[t]
 \input{defns/grad_lang/type_match}
 \caption{Type matching.}
 \label{fig:grad_lang:type-match}
\end{figure}

\begin{figure}[t]
 \input{defns/grad_lang/wf_type}
 \input{defns/grad_lang/typing}
 \caption{The type system of {\surfacelang}.}
 \label{fig:grad_lang:typing}
\end{figure}

Similar to that of {\staticlang}, the type system of {\surfacelang} consists of
two well-formedness judgments $\vdash  \Gamma$ for typing contexts and $\Gamma  \vdash  \ottnt{A}  \ottsym{:}  \ottnt{K}$ for types and a typing judgment $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$.  Their rules are shown in
\reffig{grad_lang:typing}.  There well-formedness rules are omitted because they
are the same as those of {\staticlang}, except for \WFg{Dyn}, the
well-formedness rule for the dynamic type; the full set of the inferences rules
are found in the supplementary material.  \TS{TODO; where in the material?} The
typing rules for variables \Tg{Var}, constants \Tg{Const}, functions \Tg{Lam},
type abstractions \Tg{TLam}, and the empty row \Tg{REmp} are the same as those
of {\staticlang}.  We can find that {\surfacelang} does not support a
subsumption rule for type-and-row equivalence \AI{``for''?}, and, therefore, the typing rules
are syntax-directed.

The remaining typing rules (\Tg{App}, \Tg{TApp}, \Tg{RExt}, and \Tg{RLet})
employ consistent equivalence together with \emph{type matching} $\ottnt{A}  \triangleright  \ottnt{B}$
defined by \reffig{grad_lang:type-match}, which tests if type $\ottnt{A}$ can be
supposed to be type $\ottnt{B}$.  The typing rule \Tg{App} checks that a function
$\ottnt{M}$ can have a function type $\ottnt{A_{{\mathrm{11}}}}  \rightarrow  \ottnt{A_{{\mathrm{12}}}}$ by type matching and then the
argument type $\ottnt{A_{{\mathrm{11}}}}$ is consistently equivalent to the type $\ottnt{A_{{\mathrm{2}}}}$ of an
argument $\ottnt{M_{{\mathrm{2}}}}$.  Similarly, \Tg{TApp} and \Tg{RExt} utilizes type matching to
test if a type can have forms of a universal type and a record type,
respectively.  The rule \Tg{RLet} typechecks a record decomposition that
extracts a $\ell$ field from record term $\ottnt{M_{{\mathrm{1}}}}$.  It first checks that a
$\ottnt{M_{{\mathrm{1}}}}$ can have a record type $ [  \rho  ] $ and then that $\rho$ can be
supposed to have a $\ell$ field by the row splitting operation.  If so,
\Tg{RLet} typechecks the subsequent term $\ottnt{M_{{\mathrm{2}}}}$ by using type information
obtained by the row splitting.

\TS{So..., then what?  We may be able to mention conservativity over typing of
{\staticlang} here.}

==> sections/blame_calc.tex <==
% This section is cmobination of grad_lang.otex and blame.otex

\setboolean{show-common}{true}
\setboolean{shade-common}{true}
\setboolean{show-variant}{false}
\setboolean{show-grad}{true}
\setboolean{show-grad-term}{true}
\setboolean{show-typename}{false}
\setbool{shade-dyn}{false}

\section{A polymorphic blame calculus}

\begin{figure}[t]
 \input{defns/grad_lang/syntax}
 \caption{Syntax of {\surfacelang}.}
 \label{fig:grad_lang:syntax}
\end{figure}

This section presents our language {\surfacelang}, a gradually typed counterpart
of {\staticlang} given in \sect{static_lang}.
%
% We will extend {\staticlang} and
% its counterpart with variant types in \sect{ext} after seeing how row types with
% scoped labels and row polymorphism can be handled in gradual typing through this
% and the next sections.
%
The syntax of {\surfacelang} is almost the same as that of {\staticlang}; see
\reffig{grad_lang:syntax}, where the parts shared with {\staticlang} are shaded \AI{``displayed in gray''?}.
The only difference is the addition of the dynamic type $ \star $ for value types
and row types.  The dynamic row type is just the dynamic type used in a position
requiring row types.

In the rest of this section, we present the type system of {\surfacelang}; the
semantics will be given via translation to a polymorphic blame calculus
{\interlang} in \sect{...}.  The key ingredient of the type system is
\emph{consistency}.  Consistency of {\surfacelang} is influenced by not only the
dynamic row type but also field reordering.  We first formalize consistency and
then introduce \emph{consistent equivalence} to resolve common issues of
consistency combined with subsumption like
subtyping~\cite{Siek/Taha_2007_ECOOP} \AI{What is ``subsumption like subtyping''?}.  Once we develop consistency and
consistent equivalence, the type system of {\surfacelang} is derived naturally
from that of {\staticlang}.

\subsection{Consistency}

Consistency $ \sim $ is a fundamental block of a static aspect of gradual typing
and decides possible interaction between statically typed and dynamically typed
code.  Usually, it is defined as a binary relation between types and,
intuitively, types are consistent if casts between them could
be successful.  For example, statically typed values can be injected to the
dynamic type and, conversely, dynamically typed values could be projected to any
type (whether a cast succeeds depends on whether run-time values can
behave as the target type of the cast, though).  This idea is axiomatized by the
following two rules.
\[
 \ottnt{A}  \sim  \star \qquad \star  \sim  \ottnt{A}
\]
Consistency is also defined so that type constructors are compatible with it.
For example, a consistency rule for function types is:
\[
 \frac{\ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad \ottnt{B_{{\mathrm{1}}}}  \sim  \ottnt{B_{{\mathrm{2}}}}}{\ottnt{A_{{\mathrm{1}}}}  \rightarrow  \ottnt{A_{{\mathrm{2}}}}  \sim  \ottnt{B_{{\mathrm{1}}}}  \rightarrow  \ottnt{B_{{\mathrm{2}}}}}
\]

In what follows, we discuss how to extend consistency to deal with row types and
universal types and then give its formal definition.  While that definition is
reasonable, it causes issues on typechecking and semantics.  These issues
motivate us to introduce consistent equivalence.

\subsubsection{Consistency for row types}
%
A trivial extension of consistency to row types is to allow relating the dynamic
row type to any row type ($\rho  \sim  \star$ and $\star  \sim  \rho$) and to add the
following compatible rule for row extension.
\[
  \frac{\ottnt{A}  \sim  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim    \ell  \mathbin{:}  \ottnt{B}   ;  \rho_{{\mathrm{2}}} }
\]
This rule makes, e.g., $\ottsym{(}    \ell  \mathbin{:}   \mathsf{int}    ;   \cdot    \ottsym{)}$ and $\ottsym{(}    \ell  \mathbin{:}  \star   ;   \cdot    \ottsym{)}$ consistent.

While necessary and reasonable, this compatibility rule is not sufficient to
contain all pairs of row types such that casts between them could
be successful.  The problem is in a case that row types to be related end with
$ \star $ (i.e., they take the form $  \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A_{{\mathrm{1}}}}   ;  ...  ;    \ell_{\ottmv{n}}  \mathbin{:}  \ottnt{A_{\ottmv{n}}}   ;  \star  $)
and they hold field labels distinct from those of each other.  For example, let
us consider row types $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.  While these row types are not consistent only with the above extension
of consistency, it is desirable that they are consistent because casts
between record types and between variant types with these row types could be
successful: casts between record types $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   ] $ and
$ [    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   ] $ could be successful because a record value of either of
<<<<<<< HEAD
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields \AI{Remove ``fields''?}; similarly, type conversion
=======
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields; similarly, casts
>>>>>>> master
between variant types $ \langle    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \rangle $ and $ \langle    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \rangle $
could be successful because they accommodate both of values injected with
$\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$.  It is notable that the assumption that $\ell_{{\mathrm{1}}}$ and
$\ell_{{\mathrm{2}}}$ are different labels is critical here;
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;  \star $ should not be consistent since the
types $ \mathsf{int} $ and $ \mathsf{str} $ of their $\ell$ fields are inconsistent.
\AI{More elaboration? $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;   \cdot     ] $. }

The example showing insufficiency of the simple extension above gives a
guideline to design a new consistency rule for row extension: given consistent
row types $\rho_{{\mathrm{1}}}$ and $\rho_{{\mathrm{2}}}$, extension of $\rho_{{\mathrm{1}}}$ with label $\ell$
preserves consistency with $\rho_{{\mathrm{2}}}$ if $\rho_{{\mathrm{2}}}$ ends with $ \star $ and $\ell$
does not appear in $\rho_{{\mathrm{2}}}$ .  Formally:
\[
 \frac{\quad  \rho_{{\mathrm{2}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim  \rho_{{\mathrm{2}}}}
\]
where $\mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)}$ is the set of the field labels of $\rho_{{\mathrm{2}}}$.  This rule is
justified by the intuition that: first, the occurrence of $ \star $ in $\rho_{{\mathrm{2}}}$
allows assuming that $\rho_{{\mathrm{2}}}$ could contain a field of $ \ell  \mathbin{:}  \star $; and
then the $\ell$ field can move to the head of $\rho_{{\mathrm{2}}}$ by type-and-row
equivalence since $\rho_{{\mathrm{2}}}$ is assumed not to have other $\ell$ fields.
We can apply the same discussion for extension of $\rho_{{\mathrm{2}}}$:
\[
 \frac{\quad  \rho_{{\mathrm{1}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{1}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{\rho_{{\mathrm{1}}}  \sim    \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{2}}} }
\]
Use of these two rules make row types $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \ottsym{)}$ consistent.


\subsubsection{Consistency for universal types}
%
Consistency for universal types in this work follows the earlier work on
polymorphic gradual typing by \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}.
Their consistency relates not only a universal type to another one but also a
universal type to what they call a non-$\forall$ type (i.e., a type such that
its top type constructor is not $\forall$).  The flexibility of their
consistency enables interaction between statically typed code with polymorphism
and dynamically typed code without polymorphism.  For example, in their work,
universal type $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ is consistent with non-$\forall$ type
$\star  \rightarrow  \star$.  Igarashi et al.\ present a few conditions on non-$\forall$
types to be consistent with universal types; non-$\forall$ types satisfying the
conditions are called \emph{quasi}-universal types\footnote{{Igarashi et al.}
call such types quasi-polymorphic types, but we use that term for consistent use
of terminology.} because they are not actual universal types but could behave as
them by casts.  We adjust their notion of quasi-universal
types to our setting with row types.
%
\input{defns/grad_lang/quasi-universal}
%
Then, we introduce a consistency rule like:
\[
 \frac{\quad \mathbf{QPoly} \, \ottsym{(}  \ottnt{A_{{\mathrm{2}}}}  \ottsym{)} \quad \mathit{X} \,  \not\in  \,  \mathit{ftv}  (  \ottnt{A_{{\mathrm{2}}}}  )  \quad \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad}{ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}}}
\]
and its symmetric version.

We make a remark on other choices of consistency for universal types.
\citet{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP}
give \emph{compatibility} instead of consistency.  Their compatibility is
designed to capture as many possibly successful casts as
possible, and, as a result, it deems even perhaps apparently incompatible
types---e.g., $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ and $ \mathsf{int}   \rightarrow   \mathsf{str} $---compatible.  In return for
this great flexibility, their calculus lacks conservativity over typing of
System F, the underlying calculus of their gradually typed language (i.e., a
static typing error found by System F may not be found by their gradual type
system).  Another definition of consistency is also given by
\citet{Toro/Labrada/Tanter_2019_POPL}.  Their consistency relates a universal
type only to another universal type and not to any non-$\forall$ type.  Their
gradually typed language achieves conservativity over typing of System F, but
that \AI{the?} strict distinction between universal types and non-$\forall$ types
disallows dynamically typed code, where no type information appears, to use
polymorphic values.  For example, let us consider a program $\ottnt{M} \defeq
 \lambda\!  \,  \mathit{f}  \mathord{:}  \star   \ottsym{.}  \mathit{f} \,  0 $, which calls function $\mathit{f}$ of the dynamic type $ \star $ with
integer $\ottsym{0}$.  In Toro et al.'s language, any application of $\ottnt{M}$ to a
polymorphic function would raise an exception:
\[
 \ottnt{M} \, \ottsym{(}   \Lambda\!  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \,  \lambda\!  \,  \mathit{x}  \mathord{:}  \mathit{X}   \ottsym{.}  \mathit{x}  \ottsym{)}  \longrightarrow^{*}  \mathsf{blame} \, \ottnt{p}
\]
because polymorphic values can be used successfully only if it is applied to
types.  This means that polymorphic values cannot be used in dynamically typed
code because it should have no type information including type application.

We adopt the consistency style of \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}
\AI{``The consistency style'' doesn't make sense.}
because of its balance between flexibility---it allows dynamically typed code to
use polymorphic values---and strictness \AI{I'm not sure ``strict''/''strictness'' is a right word.}---it makes a gradually typed language
conservative over typing of System F.  However, we believe that how to deal with
universal types in consistency is orthogonal to consistency for row types and
that we can choose a suitable treatment depending on a case.
\AI{cases?}


\subsubsection{Formal definition}
%
Now, we present a formal definition of consistency for {\surfacelang}.  We start
with formalizing the notions used in the consistency rules for row extension.
%
\input{defns/grad_lang/labels_in_row}
\input{defns/grad_lang/row_concat}
\input{defns/grad_lang/row_ends_with_dyn}
\AI{Do you have to define ``ending with $ \star $'' in terms of concatenation?
I thought you could define as a simple recursively defined predicate.}

We say that a relation between types is compatible if and only if it is closed
under type and row constructors.

\begin{figure}[t]
 \input{defns/grad_lang/consistency}
 \caption{Consistency.}
 \label{fig:grad_lang:consistency}
\end{figure}

\begin{defn}[Consistency]
 Consistency $\ottnt{A}  \sim  \ottnt{B}$ is the smallest compatible relation satisfying the
 rules given by \reffig{grad_lang:consistency}.
\end{defn}

\subsubsection{Issues of consistency combined with type-and-row equivalence}
\label{sec:consistency-issue}
%
Consistency does not subsume type-and-row equivalence.  Thus, if {\surfacelang}
incorporated consistency directly, it would be used combined with type-and-row
equivalence, especially in the form of composition $ \equiv  \circ  \sim $.
However, use of that composition gives rise to two issues, which were first
found in the work on gradual typing for subtyping~\cite{Siek/Taha_2007_ECOOP}.
The first issue is on typechecking.  If {\surfacelang} incorporated consistency
in the form of the composition, its typechecking algorithm would have to decide
whether given two types $\ottnt{A}$ and $\ottnt{B}$ are contained in the
composition. Thus, it would need to find an intermediate type $\ottnt{C}$ such that
$\ottnt{A}  \equiv  \ottnt{C}$ and $\ottnt{C}  \sim  \ottnt{B}$.  But, how?  This issue may not be as serious as the
case of subtyping~\cite{Siek/Taha_2007_ECOOP} because $ \equiv $ just reorders
fields in a row, but it should be still resolved.  The second issue is
more serious: incoherent semantics.  For example, let us consider the
following term
\[
\ottnt{M} \defeq \ottsym{\{}  \ell_{{\mathrm{1}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}  \ottsym{;}  \ottsym{\{}  \ell_{{\mathrm{2}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}  \ottsym{;}  \ottsym{\{}  \ottsym{\}}  \ottsym{\}}  \ottsym{\}}  \ottsym{:}  \star
\]
where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$, $\ottnt{M_{{\mathrm{1}}}}$ is a divergent term, and $\ottnt{M_{{\mathrm{2}}}}$ is a term
raising an exception (we write $\ottnt{M'}  \ottsym{:}  \ottnt{A}$ for ascription, which is a shorthand
of $\ottsym{(}   \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \mathit{x}  \ottsym{)} \, \ottnt{M'}$).  Similar to the earlier calculi for polymorphic gradual
typing~\cite{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP,Igarashi/Sekiyama/Igarashi_2017_ICFP},
evaluation of this term in {\surfacelang} would trigger application of
$ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ or $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$ to $ \star $.  \AI{Is it so clear that such an application takes place?}  But, which?  If $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ were \AI{Why subjunctive mood?}
applied, the evaluation result would be divergence; otherwise, if $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$
were, the result would be a failure of run-time checking.  Actually, which is
chosen would be determined by intermediate type $\rho$ that proves $ [    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     ]   \equiv   [  \rho  ] $ and $ [  \rho  ]   \sim  \star$ in a typing
derivation for $\ottnt{M}$, because translation of a gradually typed term to a blame
calculus depends on instances of consistency found in the
derivation~\cite{Siek/Taha_2006_SFPW}.  The problem here is that $\rho$ cannot
be determined to be unique: both of $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ can be chosen.  Although we might be able to design
coherent semantics with respect to field reordering, we take an approach more
standard in gradual
typing~\cite{Siek/Taha_2007_ECOOP,Xie/Bi/Oliveira_2018_ESOP}.

\subsection{Consistent equivalence}

To resolve the issues on consistency, we give \emph{consistent equivalence}
$ \simeq $, which characterizes composition of consistency and type-and-row
equivalence.  Our idea is to extend the consistency rules for row
extension---\Cns{ConsL} and \Cns{ConsR}---so that both cases that a label used
for extension on one side does and does not appear in a row on the other side
are taken into account; consistency handles only the latter case.  A promising
rule that handles only the former case is like:
\[
 \frac{\rho_{{\mathrm{2}}}  \equiv    \ell  \mathbin{:}  \ottnt{B}   ;  \rho'_{{\mathrm{2}}}  \quad \ottnt{A}  \simeq  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho'_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}}
\]
We merge this rule and \Cns{ConsL} into a single rule as follows.  First, we
split $\rho_{{\mathrm{2}}}$ into the first field labeled with $\ell$ and the remaining row;
these field and row correspond to $ \ell  \mathbin{:}  \ottnt{B} $ and $\rho'_{{\mathrm{2}}}$ in the rule above,
respectively.  Even in the case that $\rho_{{\mathrm{2}}}$ includes no field labeled with
$\ell$, \emph{if $\rho_{{\mathrm{2}}}$ ends with $ \star $}, then we can \emph{suppose} that
$\rho_{{\mathrm{2}}}$ includes a $\ell$ field because the dynamic row type can be supposed
to be any row type.  Since we have no idea about a type of such a $\ell$ field,
we regard it as the dynamic type conservatively.  Finally, we check consistency
between $\ottnt{A}$ and the type of the $\ell$ field extracted from $\rho_{{\mathrm{2}}}$ and
between $\rho_{{\mathrm{1}}}$ and the remaining row.

\begin{figure}[t]
 \input{defns/grad_lang/consistent_equiv}
 \caption{Consistent equivalence.}
 \label{fig:grad_lang:consistent-equiv}
\end{figure}

The idea above to merge is formalized by the consistent equivalence rule
\CE{ConsL} in \reffig{grad_lang:consistent-equiv}; there \CE{ConsR} is the
symmetric version of \CE{ConsL} and other rules have the same form as the
corresponding rules for consistency.
%
In \CE{ConsL} and \CE{ConsR}, $\rho_{{\mathrm{1}}} \,  \triangleright _{ \ell }  \, \ottnt{A}  \ottsym{,}  \rho_{{\mathrm{2}}}$ is a formalization of the
``split'' operation on row types, defined as follows.
%
\input{defns/grad_lang/row_split}
%
\begin{defn}[Consistent equivalence]
 Consistent equivalence $\ottnt{A}  \simeq  \ottnt{B}$ is the smallest compatible relation
 satisfying the rules given by \reffig{grad_lang:consistent-equiv}.
\end{defn}

We can confirm that consistent equivalence subsumes both consistency and
type-and-row equivalence by examples.  For example,
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \simeq    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ and
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ are derivable if $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.
More generally, it subsumes the composition of consistency and type-and-row
equivalence.  We can show (and actually showed) that $ \simeq $ coincides with
$ \equiv  \circ  \simeq $, but, following \citet{Xie/Bi/Oliveira_2018_ESOP}, we prove
another form of equivalence between $ \simeq $ and combination of $ \equiv $ and
$ \simeq $; the statement in this form expects us to incorporate implicit
higher-order polymorphism easily.
%
\begin{theorem}
 \label{thm:consistent-eq-consistent-equiv}
 $\ottnt{A}  \simeq  \ottnt{B}$ if and only if $\ottnt{A}  \equiv  \ottnt{A'}$ and $\ottnt{A'}  \sim  \ottnt{B'}$ and $\ottnt{B'}  \equiv  \ottnt{B}$
 for some $\ottnt{A'}$ and $\ottnt{B'}$.
\end{theorem}

We will develop the type system of {\surfacelang} using consistent equivalence in
\sect{grad_lang:typing}.  The type system does not rest on consistency, so it
does not cause the issues on typechecking nor semantics raised by consistency.
%
A typechecking algorithm for the type system does not need to infer an
intermediate type because it is enough to check if given two types are in a
single relation, consistent equivalence.  At first glance, one might consider
that it is problematic that some consistent equivalence rules are not
syntax-directed.  For example, when we would like to derive
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$, it may appear unclear which
rule of \CE{ConsL} and \CE{ConsR} should be applied first.  Fortunately, either
is fine, which is shown by the following lemma together with symmetry of
consistent subtyping.
%
\begin{lemma}%{consistent-inv-cons}
 If $  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}$,
 then $\rho_{{\mathrm{2}}} \,  \triangleright _{ \ell }  \, \ottnt{B}  \ottsym{,}  \rho'_{{\mathrm{2}}}$ and $\ottnt{A}  \simeq  \ottnt{B}$ and $\rho_{{\mathrm{1}}}  \simeq  \rho'_{{\mathrm{2}}}$.
\end{lemma}
%
For semantics, use of consistent subtyping makes the typing rules
syntax-directed, and, therefore, derivations for a typing judgment are
determined uniquely.


\subsection{Type system}
\label{sec:grad_lang:typing}

\begin{figure}[t]
 \input{defns/grad_lang/type_match}
 \caption{Type matching.}
 \label{fig:grad_lang:type-match}
\end{figure}

\begin{figure}[t]
 \input{defns/grad_lang/wf_type}
 \input{defns/grad_lang/typing}
 \caption{The type system of {\surfacelang}.}
 \label{fig:grad_lang:typing}
\end{figure}

Similar to that of {\staticlang}, the type system of {\surfacelang} consists of
two well-formedness judgments $\vdash  \Gamma$ for typing contexts and $\Gamma  \vdash  \ottnt{A}  \ottsym{:}  \ottnt{K}$ for types and a typing judgment $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$.  Their rules are shown in
\reffig{grad_lang:typing}.  There well-formedness rules are omitted because they
are the same as those of {\staticlang}, except for \WFg{Dyn}, the
well-formedness rule for the dynamic type; the full set of the inferences rules
are found in the supplementary material.  \TS{TODO; where in the material?} The
typing rules for variables \Tg{Var}, constants \Tg{Const}, functions \Tg{Lam},
type abstractions \Tg{TLam}, and the empty row \Tg{REmp} are the same as those
of {\staticlang}.  We can find that {\surfacelang} does not support a
subsumption rule for type-and-row equivalence \AI{``for''?}, and, therefore, the typing rules
are syntax-directed.

The remaining typing rules (\Tg{App}, \Tg{TApp}, \Tg{RExt}, and \Tg{RLet})
employ consistent equivalence together with \emph{type matching} $\ottnt{A}  \triangleright  \ottnt{B}$
defined by \reffig{grad_lang:type-match}, which tests if type $\ottnt{A}$ can be
supposed to be type $\ottnt{B}$.  The typing rule \Tg{App} checks that a function
$\ottnt{M}$ can have a function type $\ottnt{A_{{\mathrm{11}}}}  \rightarrow  \ottnt{A_{{\mathrm{12}}}}$ by type matching and then the
argument type $\ottnt{A_{{\mathrm{11}}}}$ is consistently equivalent to the type $\ottnt{A_{{\mathrm{2}}}}$ of an
argument $\ottnt{M_{{\mathrm{2}}}}$.  Similarly, \Tg{TApp} and \Tg{RExt} utilizes type matching to
test if a type can have forms of a universal type and a record type,
respectively.  The rule \Tg{RLet} typechecks a record decomposition that
extracts a $\ell$ field from record term $\ottnt{M_{{\mathrm{1}}}}$.  It first checks that a
$\ottnt{M_{{\mathrm{1}}}}$ can have a record type $ [  \rho  ] $ and then that $\rho$ can be
supposed to have a $\ell$ field by the row splitting operation.  If so,
\Tg{RLet} typechecks the subsequent term $\ottnt{M_{{\mathrm{2}}}}$ by using type information
obtained by the row splitting.

\TS{So..., then what?  We may be able to mention conservativity over typing of
{\staticlang} here.}

==> sections/ext.tex <==
\section{Extension with variant types}

\subsection{Syntax}

\paragraph{Types.}
%
Variant type $ \langle    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{bool}    ;   \cdot     \rangle $ is given either an integer
value tagged with $\ell_{{\mathrm{1}}}$ or a Boolean value tagged with $\ell_{{\mathrm{2}}}$.

\paragraph{Terms and values.}
%
Terms in the last line are operations on variants.  Injection $\ottsym{(}  \ell \, \ottnt{M}  \ottsym{)}$ tags
the value of $\ottnt{M}$ with label $\ell$.  The tagged values are projected by a
case expression $ \mathsf{case} \,  \ottnt{M}  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle $.  If $\ottnt{M}$ is a value
tagged with $\ell$, then the $\ottnt{M_{{\mathrm{1}}}}$ will be evaluated with the binding of
$\mathit{x}$ to the injected value; otherwise, $\ottnt{M_{{\mathrm{2}}}}$ will be with the binding of
$\mathit{y}$ to the value of $\ottnt{M}$.  At first glance, the binding of $\mathit{y}$ may
seem redundant, because $\mathit{y}$ designates the same value as $\ottnt{M}$.  However,
it is helpful to give a more precise type for the value of $\ottnt{M}$ in $\ottnt{M_{{\mathrm{2}}}}$.
Let us suppose a type of $\ottnt{M}$ to be $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;  \rho   \rangle $.  Then, the type
system of {\staticlang} allows $\mathit{y}$ to have variant type $ \langle  \rho  \rangle $ in
$\ottnt{M_{{\mathrm{2}}}}$ because we can assume in evaluation of $\ottnt{M_{{\mathrm{2}}}}$ that $\ottnt{M}$ is not
tagged with $\ell$.  We will see the detail when reviewing the type system
(\sect{static_lang:typing}).

The second variant-related operation $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} } $, called the embedding
operation~\cite{Leijen_2005_TFP}, embeds the variant value of $\ottnt{M}$ to a
variant type extended with the field of $\ell$ and $\ottnt{A}$.  Thus, for $\ottnt{M}$
of variant type $ \langle  \rho  \rangle $, $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} } $ is given type $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;  \rho   \rangle $.  In the resulting value, the label $\ell$ works as a dummy label:
the pattern for $\ell$ does not match $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} } $ and, thus, $ \mathsf{case} \,   \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} }   \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle $ will evaluate to $\ottnt{M_{{\mathrm{2}}}}$ with the
binding of $\mathit{y}$ to the value of $\ottnt{M}$.  This operation might seem not so
important for \emph{closed} row types (i.e., row types that end with the empty
row $\ottsym{(}   \cdot   \ottsym{)}$), because injection $\ell \, \ottnt{M}$ is allowed to be given variant
types that couple any label other than $\ell$ with any type\TS{and there seems
to be no practical scenario that uses duplicated labels}.  However, it could be
beneficial to \emph{open} row types (i.e., row types that end with a row
variable).  For example, let us suppose to have function $f$ of $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;  \mathit{X}   \rangle   \rightarrow  \ottnt{B}$ and variable $\mathit{x}$ of variant type $ \langle  \mathit{X}  \rangle $.  Here,
application $\mathit{f} \, \mathit{x}$ is ill typed because $\mathit{x}$ has to be of $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;  \mathit{X}   \rangle $ but not.  The embedding operation makes this application typeable by
rewriting it to $\mathit{f} \, \ottsym{(}   \variantlift{ \ell }{ \ottnt{A} }{ \mathit{x} }   \ottsym{)}$; note that other two operations on
variants--injection and case expressions---cannot resolve this.  The
practicality of the embedding operation is also investigated in the context of
algebraic effects and
handlers~\cite{Biernack/Pirog/Polesiuk/Siezkowski_2018_POPL}.

(Values are ..., or) tagged values $\ell \, \ottnt{v}$ to which the embedding operation
may be applied with $\ell$---such tagged values are denoted by $ { w }^{ \ell } $
in \reffig{static_lang:syntax}.

% a color window system, and suppose that function $f$ sets a default parser to parse a
% color string, according to the mode specified by an argument; if the mode is not
% supported, $f$ does nothing.  A possible type given to such function $f$ is:
% %
% \[
%  \texttt{\textcolor{red}{<<no parses (char 16): \mbox{$\backslash{}$}X:KR.variant <n***ame:unit,<rgb:unit,<hsv:unit,X>>> -> unit >>}}.
% \]
% %
% ($\texttt{\textcolor{red}{<<no parses (char 4): name*** >>}}$, $\texttt{\textcolor{red}{<<no parses (char 2): rg***b >>}}$, and $\texttt{\textcolor{red}{<<no parses (char 2): hs***v >>}}$ set a parser that interprets a string as a
% color name, an RGV value, and an HSV value, respectively.)

\subsection{Semantics.}
%
The rule \Rs{Embed} ignores the embedding operation if the given label $\ell$
is different from $\ell'$ with which the value is tagged.
%
The last three rules are for case expressions on variant values.  The rule
\Rs{CaseL} is applied if the label pattern of a case expression matches the
label of a tagged value; otherwise, \Rs{CaseR1} is applied.  Labels inserted by
the embedding operation are peeled off by \Rs{CaseR2}.


==> sections/grad_lang.tex <==
\setboolean{show-common}{true}
\setboolean{shade-common}{true}
\setboolean{show-variant}{false}
\setboolean{show-grad}{true}
\setboolean{show-grad-term}{true}
\setboolean{show-typename}{false}
\setbool{shade-dyn}{false}

\section{{\surfacelang}: A gradually typed counterpart of {\staticlang}}

\begin{figure}[t]
 \input{defns/grad_lang/syntax}
 \caption{Syntax of {\surfacelang}.}
 \label{fig:grad_lang:syntax}
\end{figure}

This section presents our language {\surfacelang}, a gradually typed counterpart
of {\staticlang} given in \sect{static_lang}.
%
% We will extend {\staticlang} and
% its counterpart with variant types in \sect{ext} after seeing how row types with
% scoped labels and row polymorphism can be handled in gradual typing through this
% and the next sections.
%
The syntax of {\surfacelang} is almost the same as that of {\staticlang}; see
\reffig{grad_lang:syntax}, where the parts shared with {\staticlang} are shaded \AI{``displayed in gray''?}.
The only difference is the addition of the dynamic type $ \star $ for value types
and row types.  The dynamic row type is just the dynamic type used in a position
requiring row types.

In the rest of this section, we present the type system of {\surfacelang}; the
semantics will be given via translation to a polymorphic blame calculus
{\interlang} in \sect{...}.  The key ingredient of the type system is
\emph{consistency}.  Consistency of {\surfacelang} is influenced by not only the
dynamic row type but also field reordering.  We first formalize consistency and
then introduce \emph{consistent equivalence} to resolve common issues of
consistency combined with subsumption like
subtyping~\cite{Siek/Taha_2007_ECOOP} \AI{What is ``subsumption like subtyping''?}.  Once we develop consistency and
consistent equivalence, the type system of {\surfacelang} is derived naturally
from that of {\staticlang}.

\subsection{Consistency}

Consistency $ \sim $ is a fundamental block of a static aspect of gradual typing
and decides possible interaction between statically typed and dynamically typed
code.  Usually, it is defined as a binary relation between types and,
intuitively, types are consistent if casts between them could
be successful.  For example, statically typed values can be injected to the
dynamic type and, conversely, dynamically typed values could be projected to any
type (whether a cast succeeds depends on whether run-time values can
behave as the target type of the cast, though).  This idea is axiomatized by the
following two rules.
\[
 \ottnt{A}  \sim  \star \qquad \star  \sim  \ottnt{A}
\]
Consistency is also defined so that type constructors are compatible with it.
For example, a consistency rule for function types is:
\[
 \frac{\ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad \ottnt{B_{{\mathrm{1}}}}  \sim  \ottnt{B_{{\mathrm{2}}}}}{\ottnt{A_{{\mathrm{1}}}}  \rightarrow  \ottnt{A_{{\mathrm{2}}}}  \sim  \ottnt{B_{{\mathrm{1}}}}  \rightarrow  \ottnt{B_{{\mathrm{2}}}}}
\]

In what follows, we discuss how to extend consistency to deal with row types and
universal types and then give its formal definition.  While that definition is
reasonable, it causes issues on typechecking and semantics.  These issues
motivate us to introduce consistent equivalence.

\subsubsection{Consistency for row types}
%
A trivial extension of consistency to row types is to allow relating the dynamic
row type to any row type ($\rho  \sim  \star$ and $\star  \sim  \rho$) and to add the
following compatible rule for row extension.
\[
  \frac{\ottnt{A}  \sim  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim    \ell  \mathbin{:}  \ottnt{B}   ;  \rho_{{\mathrm{2}}} }
\]
This rule makes, e.g., $\ottsym{(}    \ell  \mathbin{:}   \mathsf{int}    ;   \cdot    \ottsym{)}$ and $\ottsym{(}    \ell  \mathbin{:}  \star   ;   \cdot    \ottsym{)}$ consistent.

While necessary and reasonable, this compatibility rule is not sufficient to
contain all pairs of row types such that casts between them could
be successful.  The problem is in a case that row types to be related end with
$ \star $ (i.e., they take the form $  \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A_{{\mathrm{1}}}}   ;  ...  ;    \ell_{\ottmv{n}}  \mathbin{:}  \ottnt{A_{\ottmv{n}}}   ;  \star  $)
and they hold field labels distinct from those of each other.  For example, let
us consider row types $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.  While these row types are not consistent only with the above extension
of consistency, it is desirable that they are consistent because casts
between record types and between variant types with these row types could be
successful: casts between record types $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   ] $ and
$ [    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   ] $ could be successful because a record value of either of
<<<<<<< HEAD
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields \AI{Remove ``fields''?}; similarly, type conversion
=======
them could hold both $\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$ fields; similarly, casts
>>>>>>> master
between variant types $ \langle    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \rangle $ and $ \langle    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \rangle $
could be successful because they accommodate both of values injected with
$\ell_{{\mathrm{1}}}$ and $\ell_{{\mathrm{2}}}$.  It is notable that the assumption that $\ell_{{\mathrm{1}}}$ and
$\ell_{{\mathrm{2}}}$ are different labels is critical here;
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star $ and $  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;  \star $ should not be consistent since the
types $ \mathsf{int} $ and $ \mathsf{str} $ of their $\ell$ fields are inconsistent.
\AI{More elaboration? $ [    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{str}    ;   \cdot     ] $. }

The example showing insufficiency of the simple extension above gives a
guideline to design a new consistency rule for row extension: given consistent
row types $\rho_{{\mathrm{1}}}$ and $\rho_{{\mathrm{2}}}$, extension of $\rho_{{\mathrm{1}}}$ with label $\ell$
preserves consistency with $\rho_{{\mathrm{2}}}$ if $\rho_{{\mathrm{2}}}$ ends with $ \star $ and $\ell$
does not appear in $\rho_{{\mathrm{2}}}$ .  Formally:
\[
 \frac{\quad  \rho_{{\mathrm{2}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \sim  \rho_{{\mathrm{2}}}}
\]
where $\mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{2}}}  \ottsym{)}$ is the set of the field labels of $\rho_{{\mathrm{2}}}$.  This rule is
justified by the intuition that: first, the occurrence of $ \star $ in $\rho_{{\mathrm{2}}}$
allows assuming that $\rho_{{\mathrm{2}}}$ could contain a field of $ \ell  \mathbin{:}  \star $; and
then the $\ell$ field can move to the head of $\rho_{{\mathrm{2}}}$ by type-and-row
equivalence since $\rho_{{\mathrm{2}}}$ is assumed not to have other $\ell$ fields.
We can apply the same discussion for extension of $\rho_{{\mathrm{2}}}$:
\[
 \frac{\quad  \rho_{{\mathrm{1}}}  \text{ ends with }  \star  \quad \ell \,  \not\in  \, \mathit{dom} \, \ottsym{(}  \rho_{{\mathrm{1}}}  \ottsym{)} \quad \rho_{{\mathrm{1}}}  \sim  \rho_{{\mathrm{2}}} \quad}{\rho_{{\mathrm{1}}}  \sim    \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{2}}} }
\]
Use of these two rules make row types $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star   \ottsym{)}$ consistent.


\subsubsection{Consistency for universal types}
%
Consistency for universal types in this work follows the earlier work on
polymorphic gradual typing by \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}.
Their consistency relates not only a universal type to another one but also a
universal type to what they call a non-$\forall$ type (i.e., a type such that
its top type constructor is not $\forall$).  The flexibility of their
consistency enables interaction between statically typed code with polymorphism
and dynamically typed code without polymorphism.  For example, in their work,
universal type $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ is consistent with non-$\forall$ type
$\star  \rightarrow  \star$.  Igarashi et al.\ present a few conditions on non-$\forall$
types to be consistent with universal types; non-$\forall$ types satisfying the
conditions are called \emph{quasi}-universal types\footnote{{Igarashi et al.}
call such types quasi-polymorphic types, but we use that term for consistent use
of terminology.} because they are not actual universal types but could behave as
them by casts.  We adjust their notion of quasi-universal
types to our setting with row types.
%
\input{defns/grad_lang/quasi-universal}
%
Then, we introduce a consistency rule like:
\[
 \frac{\quad \mathbf{QPoly} \, \ottsym{(}  \ottnt{A_{{\mathrm{2}}}}  \ottsym{)} \quad \mathit{X} \,  \not\in  \,  \mathit{ftv}  (  \ottnt{A_{{\mathrm{2}}}}  )  \quad \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}} \quad}{ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{A_{{\mathrm{1}}}}  \sim  \ottnt{A_{{\mathrm{2}}}}}
\]
and its symmetric version.

We make a remark on other choices of consistency for universal types.
\citet{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP}
give \emph{compatibility} instead of consistency.  Their compatibility is
designed to capture as many possibly successful casts as
possible, and, as a result, it deems even perhaps apparently incompatible
types---e.g., $ \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \, \mathit{X}  \rightarrow  \mathit{X}$ and $ \mathsf{int}   \rightarrow   \mathsf{str} $---compatible.  In return for
this great flexibility, their calculus lacks conservativity over typing of
System F, the underlying calculus of their gradually typed language (i.e., a
static typing error found by System F may not be found by their gradual type
system).  Another definition of consistency is also given by
\citet{Toro/Labrada/Tanter_2019_POPL}.  Their consistency relates a universal
type only to another universal type and not to any non-$\forall$ type.  Their
gradually typed language achieves conservativity over typing of System F, but
that \AI{the?} strict distinction between universal types and non-$\forall$ types
disallows dynamically typed code, where no type information appears, to use
polymorphic values.  For example, let us consider a program $\ottnt{M} \defeq
 \lambda\!  \,  \mathit{f}  \mathord{:}  \star   \ottsym{.}  \mathit{f} \,  0 $, which calls function $\mathit{f}$ of the dynamic type $ \star $ with
integer $\ottsym{0}$.  In Toro et al.'s language, any application of $\ottnt{M}$ to a
polymorphic function would raise an exception:
\[
 \ottnt{M} \, \ottsym{(}   \Lambda\!  \,  \mathit{X}  \mathord{:}   \mathsf{T}    \ottsym{.} \,  \lambda\!  \,  \mathit{x}  \mathord{:}  \mathit{X}   \ottsym{.}  \mathit{x}  \ottsym{)}  \longrightarrow^{*}  \mathsf{blame} \, \ottnt{p}
\]
because polymorphic values can be used successfully only if it is applied to
types.  This means that polymorphic values cannot be used in dynamically typed
code because it should have no type information including type application.

We adopt the consistency style of \citet{Igarashi/Sekiyama/Igarashi_2017_ICFP}
\AI{``The consistency style'' doesn't make sense.}
because of its balance between flexibility---it allows dynamically typed code to
use polymorphic values---and strictness \AI{I'm not sure ``strict''/''strictness'' is a right word.}---it makes a gradually typed language
conservative over typing of System F.  However, we believe that how to deal with
universal types in consistency is orthogonal to consistency for row types and
that we can choose a suitable treatment depending on a case.
\AI{cases?}


\subsubsection{Formal definition}
%
Now, we present a formal definition of consistency for {\surfacelang}.  We start
with formalizing the notions used in the consistency rules for row extension.
%
\input{defns/grad_lang/labels_in_row}
\input{defns/grad_lang/row_concat}
\input{defns/grad_lang/row_ends_with_dyn}
\AI{Do you have to define ``ending with $ \star $'' in terms of concatenation?
I thought you could define as a simple recursively defined predicate.}

We say that a relation between types is compatible if and only if it is closed
under type and row constructors.

\begin{figure}[t]
 \input{defns/grad_lang/consistency}
 \caption{Consistency.}
 \label{fig:grad_lang:consistency}
\end{figure}

\begin{defn}[Consistency]
 Consistency $\ottnt{A}  \sim  \ottnt{B}$ is the smallest compatible relation satisfying the
 rules given by \reffig{grad_lang:consistency}.
\end{defn}

\subsubsection{Issues of consistency combined with type-and-row equivalence}
\label{sec:consistency-issue}
%
Consistency does not subsume type-and-row equivalence.  Thus, if {\surfacelang}
incorporated consistency directly, it would be used combined with type-and-row
equivalence, especially in the form of composition $ \equiv  \circ  \sim $.
However, use of that composition gives rise to two issues, which were first
found in the work on gradual typing for subtyping~\cite{Siek/Taha_2007_ECOOP}.
The first issue is on typechecking.  If {\surfacelang} incorporated consistency
in the form of the composition, its typechecking algorithm would have to decide
whether given two types $\ottnt{A}$ and $\ottnt{B}$ are contained in the
composition. Thus, it would need to find an intermediate type $\ottnt{C}$ such that
$\ottnt{A}  \equiv  \ottnt{C}$ and $\ottnt{C}  \sim  \ottnt{B}$.  But, how?  This issue may not be as serious as the
case of subtyping~\cite{Siek/Taha_2007_ECOOP} because $ \equiv $ just reorders
fields in a row, but it should be still resolved.  The second issue is
more serious: incoherent semantics.  For example, let us consider the
following term
\[
\ottnt{M} \defeq \ottsym{\{}  \ell_{{\mathrm{1}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}  \ottsym{;}  \ottsym{\{}  \ell_{{\mathrm{2}}}  \ottsym{=}   \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}  \ottsym{;}  \ottsym{\{}  \ottsym{\}}  \ottsym{\}}  \ottsym{\}}  \ottsym{:}  \star
\]
where $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$, $\ottnt{M_{{\mathrm{1}}}}$ is a divergent term, and $\ottnt{M_{{\mathrm{2}}}}$ is a term
raising an exception (we write $\ottnt{M'}  \ottsym{:}  \ottnt{A}$ for ascription, which is a shorthand
of $\ottsym{(}   \lambda\!  \,  \mathit{x}  \mathord{:}  \ottnt{A}   \ottsym{.}  \mathit{x}  \ottsym{)} \, \ottnt{M'}$).  Similar to the earlier calculi for polymorphic gradual
typing~\cite{Ahmed/Findler/Siek/Wadler_2011_POPL,Ahmed/Jamner/Siek/Wadler_2017_ICFP,Igarashi/Sekiyama/Igarashi_2017_ICFP},
evaluation of this term in {\surfacelang} would trigger application of
$ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ or $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$ to $ \star $.  \AI{Is it so clear that such an application takes place?}  But, which?  If $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{1}}}}$ were \AI{Why subjunctive mood?}
applied, the evaluation result would be divergence; otherwise, if $ \Lambda\!  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{M_{{\mathrm{2}}}}$
were, the result would be a failure of run-time checking.  Actually, which is
chosen would be determined by intermediate type $\rho$ that proves $ [    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     ]   \equiv   [  \rho  ] $ and $ [  \rho  ]   \sim  \star$ in a typing
derivation for $\ottnt{M}$, because translation of a gradually typed term to a blame
calculus depends on instances of consistency found in the
derivation~\cite{Siek/Taha_2006_SFPW}.  The problem here is that $\rho$ cannot
be determined to be unique: both of $\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}$ and
$\ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ can be chosen.  Although we might be able to design
coherent semantics with respect to field reordering, we take an approach more
standard in gradual
typing~\cite{Siek/Taha_2007_ECOOP,Xie/Bi/Oliveira_2018_ESOP}.

\subsection{Consistent equivalence}

To resolve the issues on consistency, we give \emph{consistent equivalence}
$ \simeq $, which characterizes composition of consistency and type-and-row
equivalence.  Our idea is to extend the consistency rules for row
extension---\Cns{ConsL} and \Cns{ConsR}---so that both cases that a label used
for extension on one side does and does not appear in a row on the other side
are taken into account; consistency handles only the latter case.  A promising
rule that handles only the former case is like:
\[
 \frac{\rho_{{\mathrm{2}}}  \equiv    \ell  \mathbin{:}  \ottnt{B}   ;  \rho'_{{\mathrm{2}}}  \quad \ottnt{A}  \simeq  \ottnt{B} \quad \rho_{{\mathrm{1}}}  \sim  \rho'_{{\mathrm{2}}}}{  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}}
\]
We merge this rule and \Cns{ConsL} into a single rule as follows.  First, we
split $\rho_{{\mathrm{2}}}$ into the first field labeled with $\ell$ and the remaining row;
these field and row correspond to $ \ell  \mathbin{:}  \ottnt{B} $ and $\rho'_{{\mathrm{2}}}$ in the rule above,
respectively.  Even in the case that $\rho_{{\mathrm{2}}}$ includes no field labeled with
$\ell$, \emph{if $\rho_{{\mathrm{2}}}$ ends with $ \star $}, then we can \emph{suppose} that
$\rho_{{\mathrm{2}}}$ includes a $\ell$ field because the dynamic row type can be supposed
to be any row type.  Since we have no idea about a type of such a $\ell$ field,
we regard it as the dynamic type conservatively.  Finally, we check consistency
between $\ottnt{A}$ and the type of the $\ell$ field extracted from $\rho_{{\mathrm{2}}}$ and
between $\rho_{{\mathrm{1}}}$ and the remaining row.

\begin{figure}[t]
 \input{defns/grad_lang/consistent_equiv}
 \caption{Consistent equivalence.}
 \label{fig:grad_lang:consistent-equiv}
\end{figure}

The idea above to merge is formalized by the consistent equivalence rule
\CE{ConsL} in \reffig{grad_lang:consistent-equiv}; there \CE{ConsR} is the
symmetric version of \CE{ConsL} and other rules have the same form as the
corresponding rules for consistency.
%
In \CE{ConsL} and \CE{ConsR}, $\rho_{{\mathrm{1}}} \,  \triangleright _{ \ell }  \, \ottnt{A}  \ottsym{,}  \rho_{{\mathrm{2}}}$ is a formalization of the
``split'' operation on row types, defined as follows.
%
\input{defns/grad_lang/row_split}
%
\begin{defn}[Consistent equivalence]
 Consistent equivalence $\ottnt{A}  \simeq  \ottnt{B}$ is the smallest compatible relation
 satisfying the rules given by \reffig{grad_lang:consistent-equiv}.
\end{defn}

We can confirm that consistent equivalence subsumes both consistency and
type-and-row equivalence by examples.  For example,
$  \ell_{{\mathrm{1}}}  \mathbin{:}   \mathsf{int}    ;  \star   \simeq    \ell_{{\mathrm{2}}}  \mathbin{:}   \mathsf{str}    ;  \star $ and
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$ are derivable if $\ell_{{\mathrm{1}}} \,  \not=  \, \ell_{{\mathrm{2}}}$.
More generally, it subsumes the composition of consistency and type-and-row
equivalence.  We can show (and actually showed) that $ \simeq $ coincides with
$ \equiv  \circ  \simeq $, but, following \citet{Xie/Bi/Oliveira_2018_ESOP}, we prove
another form of equivalence between $ \simeq $ and combination of $ \equiv $ and
$ \simeq $; the statement in this form expects us to incorporate implicit
higher-order polymorphism easily.
%
\begin{theorem}
 \label{thm:consistent-eq-consistent-equiv}
 $\ottnt{A}  \simeq  \ottnt{B}$ if and only if $\ottnt{A}  \equiv  \ottnt{A'}$ and $\ottnt{A'}  \sim  \ottnt{B'}$ and $\ottnt{B'}  \equiv  \ottnt{B}$
 for some $\ottnt{A'}$ and $\ottnt{B'}$.
\end{theorem}

We will develop the type system of {\surfacelang} using consistent equivalence in
\sect{grad_lang:typing}.  The type system does not rest on consistency, so it
does not cause the issues on typechecking nor semantics raised by consistency.
%
A typechecking algorithm for the type system does not need to infer an
intermediate type because it is enough to check if given two types are in a
single relation, consistent equivalence.  At first glance, one might consider
that it is problematic that some consistent equivalence rules are not
syntax-directed.  For example, when we would like to derive
$\ottsym{(}    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;   \cdot     \ottsym{)}  \simeq  \ottsym{(}    \ell_{{\mathrm{2}}}  \mathbin{:}  \ottnt{B}   ;    \ell_{{\mathrm{1}}}  \mathbin{:}  \ottnt{A}   ;   \cdot     \ottsym{)}$, it may appear unclear which
rule of \CE{ConsL} and \CE{ConsR} should be applied first.  Fortunately, either
is fine, which is shown by the following lemma together with symmetry of
consistent subtyping.
%
\begin{lemma}%{consistent-inv-cons}
 If $  \ell  \mathbin{:}  \ottnt{A}   ;  \rho_{{\mathrm{1}}}   \simeq  \rho_{{\mathrm{2}}}$,
 then $\rho_{{\mathrm{2}}} \,  \triangleright _{ \ell }  \, \ottnt{B}  \ottsym{,}  \rho'_{{\mathrm{2}}}$ and $\ottnt{A}  \simeq  \ottnt{B}$ and $\rho_{{\mathrm{1}}}  \simeq  \rho'_{{\mathrm{2}}}$.
\end{lemma}
%
For semantics, use of consistent subtyping makes the typing rules
syntax-directed, and, therefore, derivations for a typing judgment are
determined uniquely.


\subsection{Type system}
\label{sec:grad_lang:typing}

\begin{figure}[t]
 \input{defns/grad_lang/type_match}
 \caption{Type matching.}
 \label{fig:grad_lang:type-match}
\end{figure}

\begin{figure}[t]
 \input{defns/grad_lang/wf_type}
 \input{defns/grad_lang/typing}
 \caption{The type system of {\surfacelang}.}
 \label{fig:grad_lang:typing}
\end{figure}

Similar to that of {\staticlang}, the type system of {\surfacelang} consists of
two well-formedness judgments $\vdash  \Gamma$ for typing contexts and $\Gamma  \vdash  \ottnt{A}  \ottsym{:}  \ottnt{K}$ for types and a typing judgment $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$.  Their rules are shown in
\reffig{grad_lang:typing}.  There well-formedness rules are omitted because they
are the same as those of {\staticlang}, except for \WFg{Dyn}, the
well-formedness rule for the dynamic type; the full set of the inferences rules
are found in the supplementary material.  \TS{TODO; where in the material?} The
typing rules for variables \Tg{Var}, constants \Tg{Const}, functions \Tg{Lam},
type abstractions \Tg{TLam}, and the empty row \Tg{REmp} are the same as those
of {\staticlang}.  We can find that {\surfacelang} does not support a
subsumption rule for type-and-row equivalence \AI{``for''?}, and, therefore, the typing rules
are syntax-directed.

The remaining typing rules (\Tg{App}, \Tg{TApp}, \Tg{RExt}, and \Tg{RLet})
employ consistent equivalence together with \emph{type matching} $\ottnt{A}  \triangleright  \ottnt{B}$
defined by \reffig{grad_lang:type-match}, which tests if type $\ottnt{A}$ can be
supposed to be type $\ottnt{B}$.  The typing rule \Tg{App} checks that a function
$\ottnt{M}$ can have a function type $\ottnt{A_{{\mathrm{11}}}}  \rightarrow  \ottnt{A_{{\mathrm{12}}}}$ by type matching and then the
argument type $\ottnt{A_{{\mathrm{11}}}}$ is consistently equivalent to the type $\ottnt{A_{{\mathrm{2}}}}$ of an
argument $\ottnt{M_{{\mathrm{2}}}}$.  Similarly, \Tg{TApp} and \Tg{RExt} utilizes type matching to
test if a type can have forms of a universal type and a record type,
respectively.  The rule \Tg{RLet} typechecks a record decomposition that
extracts a $\ell$ field from record term $\ottnt{M_{{\mathrm{1}}}}$.  It first checks that a
$\ottnt{M_{{\mathrm{1}}}}$ can have a record type $ [  \rho  ] $ and then that $\rho$ can be
supposed to have a $\ell$ field by the row splitting operation.  If so,
\Tg{RLet} typechecks the subsequent term $\ottnt{M_{{\mathrm{2}}}}$ by using type information
obtained by the row splitting.

\TS{So..., then what?  We may be able to mention conservativity over typing of
{\staticlang} here.}

==> sections/prop.tex <==
\section{Properties}
\label{sec:prop}

This section states properties of {\surfacelang} and {\interlang}; their
detailed proofs are found in the supplementary material.  In this section, we
consider languages {\staticlang}, {\surfacelang}, and {\interlang} extended with
variants in \sect{variant}.

We start with showing type soundness of {\surfacelang}, which rest on two
theorems: type preservation of the translation from {\surfacelang} to
{\interlang} and type soundness of {\interlang}.  In what follows, $ { \makestatic{\longrightarrow} }^{*} $
is the transitive closure of $ \makestatic{\longrightarrow} $; $ \Sigma  \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma'  \mid  \ottnt{e'} $ denotes a
sequence of $ \Sigma  \mid  \ottnt{e}   \longrightarrow   \Sigma_{{\mathrm{0}}}  \mid  \ottnt{e_{{\mathrm{0}}}} $, ..., $ \Sigma_{\ottmv{n}}  \mid  \ottnt{e_{\ottmv{n}}}   \longrightarrow   \Sigma'  \mid  \ottnt{e'} $; and
$ \Sigma  \mid  \ottnt{e}   \centernot\longrightarrow$ means that there are no $\Sigma'$ and $\ottnt{e'}$ such that
$ \Sigma  \mid  \ottnt{e}   \longrightarrow   \Sigma'  \mid  \ottnt{e'} $.
%
\begin{theorem}[Type preservation of translation]
 Assume that $\ottnt{C}  \oplus  \ottnt{D}$ is consistently equivalent to both $\ottnt{C}$ and
 $\ottnt{D}$.
 %
 If $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$ and $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}  \hookrightarrow  \ottnt{e}$, then $ \emptyset   \ottsym{;}  \Gamma  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}$.
 \TS{TODO}
\end{theorem}
\noindent
%
Type soundness of {\interlang} is shown by progress and subject reduction.
%
\begin{lemma}[Progress] \label{ref:progress}
 If $\Sigma  \ottsym{;}   \emptyset   \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}$, then one of the followings holds:
 %
 (1) $\ottnt{e}$ is a value; (2) $\ottnt{e} \,  =  \, \mathsf{blame} \, \ottnt{p}$ for some $\ell$; or
 (3) $ \Sigma  \mid  \ottnt{e}   \longrightarrow   \Sigma'  \mid  \ottnt{e'} $ for some $\Sigma'$ and $\ottnt{e'}$.
\end{lemma}
%
\begin{lemma}[Subject reduction] \label{lem:subject-red}
 If $\Sigma  \ottsym{;}   \emptyset   \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}$ and $ \Sigma  \mid  \ottnt{e}   \longrightarrow   \Sigma'  \mid  \ottnt{e'} $,
 then $\Sigma'  \ottsym{;}   \emptyset   \vdash  \ottnt{e'}  \ottsym{:}  \ottnt{A}$.
\end{lemma}
%
\begin{theorem}[Type soundness of {\surfacelang}]
 If $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$ and $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}  \hookrightarrow  \ottnt{e}$ and $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma'  \mid  \ottnt{e'} $
 and $ \Sigma'  \mid  \ottnt{e'}   \centernot\longrightarrow$, then either $\ottnt{e'}$ is a value or $\ottnt{e'} \,  =  \, \mathsf{blame} \, \ottnt{p}$
 for some $\ottnt{p}$.
\end{theorem}

We also show that {\surfacelang} is a conservative extension of {\staticlang}
over both typing and semantics.
%
\begin{theorem}[Convervativity]
 \TS{TODO}
 Suppose $ \star $ does not appear in $\Gamma$, $\ottnt{M}$, and $\ottnt{A}$.
 \begin{itemize}
  \item $ \Gamma  \mathrel{ \makestatic{\vdash} }  \ottnt{M}  :  \ottnt{A} $ if and only if $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$.
  \item Suppose that $ \emptyset   \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$ and $ \emptyset   \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}  \hookrightarrow  \ottnt{e}$.
        Then, $ \ottnt{M}  \mathrel{ { \makestatic{\longrightarrow} }^{*} }  w $ if and only if $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \ottnt{v} $.
 \end{itemize}
\end{theorem}

Finally, we state the gradual guarantee property of {\surfacelang}, which
formalizes the intuition that use of more static types (i.e., types where
$ \star $ occurs less frequently) does not change the behavior of programs in
terms of both typing and semantics except that the programs with more static
types may give rise to more typing errors and
exceptions~\cite{Siek/Vitousek/Cimini/Boyland_2015_SNAPL}.  The notion of ``use
of more static types'' is represented by so-called \emph{precision} $ \sqsubseteq $,
which is defined usually to be the smallest relation between types satisfying
$\ottnt{A} \, \sqsubseteq \, \star$.  However, it is known that gradual guarantee with precision
defined in this way does not hold in polymorphic gradual
typing~\cite{Igarashi/Sekiyama/Igarashi_2017_ICFP,Toro/Labrada/Tanter_2019_POPL}.
The crux of the problem is in universal types, especially, related to $ \star $
by precision.  To avoid this problem, precision dealt with by this paper relates
a universal type only to another universal type and not to $ \star $.  We show
gradual guarantee with precision defined in such a way.
%
\begin{defn}[Precision]
 \TS{TODO}
 Type precision $\ottnt{A} \, \sqsubseteq \, \ottnt{B}$ is the smallest compatible relation satisfying:
 \[
  \frac{\ottnt{A} \,  \not=  \,  \text{\unboldmath$\forall\!$}  \,  \mathit{X}  \mathord{:}  \ottnt{K}   \ottsym{.} \, \ottnt{B}}{\ottnt{A} \, \sqsubseteq \, \star}
 \]
 Term precision $\ottnt{M_{{\mathrm{1}}}} \, \sqsubseteq \, \ottnt{M_{{\mathrm{2}}}}$ is defined if and only if $\ottnt{M_{{\mathrm{1}}}}$ and $\ottnt{M_{{\mathrm{2}}}}$
 are equivalent up to corresponding type annotations and the pairs of the
 annotations are contained in type precision.
\end{defn}
%
\begin{theorem}[Gradual guarantee]
 \TS{TODO}
 If $\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$ and $\ottnt{M} \, \sqsubseteq \, \ottnt{M'}$, then $\Gamma  \vdash  \ottnt{M'}  \ottsym{:}  \ottnt{A'}$ and $\ottnt{A} \, \sqsubseteq \, \ottnt{A'}$
 for some $\ottnt{A}$.
 %
 Furthermore, suppose that $\Gamma \,  =  \,  \emptyset $ and $ \emptyset   \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}  \hookrightarrow  \ottnt{e}$ and
 $ \emptyset   \vdash  \ottnt{M'}  \ottsym{:}  \ottnt{A'}  \hookrightarrow  \ottnt{e'}$.  Then:
 \begin{itemize}
  \item[(1a)] If $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \ottnt{v} $, then $  \emptyset   \mid  \ottnt{e'}   \longrightarrow^{*}   \Sigma'  \mid  \ottnt{v'} $ \TS{and $\ottnt{v}$ prec $\ottnt{v'}$}
              for some $\Sigma'$ and $\ottnt{v'}$.
  \item[(1b)] If $\ottnt{e}$ diverges, so does $\ottnt{e'}$.
  \item[(2a)] If $  \emptyset   \mid  \ottnt{e'}   \longrightarrow^{*}   \Sigma'  \mid  \ottnt{v'} $,
              then $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \ottnt{v} $ \TS{and $\ottnt{v}$ prec $\ottnt{v'}$} for some $\Sigma$ and $\ottnt{v}$,
              or $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \mathsf{blame} \, \ottnt{p} $ for some $\Sigma$ and $\ottnt{p}$.
  \item[(2b)] If $  \emptyset   \mid  \ottnt{e'}   \longrightarrow^{*}   \Sigma'  \mid  \mathsf{blame} \, \ottnt{p} $,
              then $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \mathsf{blame} \, \ottnt{q} $ for some $\Sigma$ and $\ottnt{q}$.
  \item[(2c)] If $\ottnt{e'}$ diverges, so does $\ottnt{e}$ or $  \emptyset   \mid  \ottnt{e}   \longrightarrow^{*}   \Sigma  \mid  \mathsf{blame} \, \ottnt{p} $ for some $\Sigma$ and $\ottnt{p}$.
 \end{itemize}
\end{theorem}


==> sections/variant.tex <==
\setboolean{show-common}{false}
\setboolean{show-variant}{true}

\section{Extension with variant types}
\label{sec:variant}

This section extends languages {\staticlang}, {\surfacelang}, and {\interlang}
with variants.  We show only the key parts of the extensions; the full versions
of the extended languages are found in the supplementary material. \TS{TODO}.

\subsection{Variants, statically typed}

\begin{figure}[t]
 % syntax
 \[\begin{array}{lrl}
  \syntax-type-row{} \\[.5ex]
  \syntaxMterm{}
  \syntaxWvalue{}
  \syntaxFctx{}
 \end{array}\]
 %
 % semantics
 \begin{flushleft}
  \input{defns/static_lang/reduction}
 \end{flushleft}
 %
 % type system
 \begin{flushleft}
  \textbf{Typing and well-formedness rules} \quad
  \framebox{$ \mathrel{ \makestatic{\vdash} }  \Gamma $} \quad
  \framebox{$ \Gamma  \mathrel{ \makestatic{\vdash} }  \ottnt{A}  :  \ottnt{K} $} \quad
  \framebox{$ \Gamma  \mathrel{ \makestatic{\vdash} }  \ottnt{M}  :  \ottnt{A} $}
 \end{flushleft}
 \begin{center}
  \input{defns/static_lang/wf_type_rules} \vspace{3ex}
  \input{defns/static_lang/typing_rules}
 \end{center}
 \caption{The extension of {\staticlang} with variants.}
 \label{fig:variant:static_lang}
\end{figure}

The extension of {\staticlang} with variants is shown in
\reffig{variant:static_lang}.

\paragraph{Syntax}
Types are extended with variant types $ \langle  \rho  \rangle $, which inhabit values
tagged with field labels in $\rho$.
%
Terms have three new constructors for variants.  Injection $\ottsym{(}  \ell \, \ottnt{M}  \ottsym{)}$ tags the
value of $\ottnt{M}$ with $\ell$.  Embedding term $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} } $ embeds the
value of $\ottnt{M}$ into a variant type extended with field $ \ell  \mathbin{:}  \ottnt{A} $.  If $\ottnt{M}$
is an injection with $\ell$, the embedding ``shadows'' the injection.  Case
expression $ \mathsf{case} \,  \ottnt{M}  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle $, where $\mathit{x}$ and $\mathit{y}$ are
bound in $\ottnt{M_{{\mathrm{1}}}}$ and $\ottnt{M_{{\mathrm{2}}}}$, tests the variant value of $\ottnt{M}$ on $\ell$.
%
% If it is an injection with $\ell$, $\ottnt{M_{{\mathrm{1}}}}$ will be evaluated with the binding
% of $\mathit{x}$ to the injected value; otherwise, $\ottnt{M_{{\mathrm{2}}}}$ will be evaluated with the
% biding of $\mathit{y}$ to the variant value obtained by peeling off the first label
% $\ell$ from the value of $\ottnt{M}$.
%
Variant values, ranged over by $ { w }^{ \ell } $, are injections on which zero or
more applications of the embedding constructor are stacked with the same labels
as the underlying injections.
%
Evaluation contexts $F$ are extended just in accordance with the extension
of terms.

\paragraph{Semantics}
The semantics is extended with four reduction rules.  The first is for embedding
terms and it means that embedding is discarded if labels held by an embedding
term and an underlying injection are different.  The other three rules are for
case expressions $ \mathsf{case} \,   { w }^{ \ell' }   \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle $.  If $ { w }^{ \ell' } $ is an injection with $\ell$, the branch $\ottnt{M_{{\mathrm{1}}}}$ will be evaluated with
substitution of the injected value for $\mathit{x}$ \Rs{CaseL}.  If $ { w }^{ \ell' } $
is an embedding term with $\ell$, the top embedding constructor is popped from
the stack and the underlying variant value is substituted for $\mathit{y}$ in
$\ottnt{M_{{\mathrm{2}}}}$ \Rs{CaseR1}.  If $\ell \,  \not=  \, \ell'$, $\ottnt{M_{{\mathrm{2}}}}$ will be evaluated with
substitution of the same variant value for $\mathit{y}$ \Rs{CaseR2}.

\paragraph{Type system}
%
The type system is augmented with a well-formedness rule for record types and
typing rules for injection, embedding, and case matching on labels.  Injection
$\ell \, \ottnt{M}$ can be given any variant type of which the first $\ell$ field has the
same type as $\ottnt{M}$.  Embedding $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{M} } $ shadows $\ell$ fields in the
variant type of $\ottnt{M}$.  For case expression $ \mathsf{case} \,  \ottnt{M}  \,\mathsf{with}\, \langle  \ell \,  \mathit{x}   \rightarrow   \ottnt{M_{{\mathrm{1}}}}   \ottsym{;}   \mathit{y}   \rightarrow   \ottnt{M_{{\mathrm{2}}}}  \rangle $, matched expression $\ottnt{M}$ must have a variant type holding an $\ell$
field.  Branches $\ottnt{M_{{\mathrm{1}}}}$ and $\ottnt{M_{{\mathrm{2}}}}$ are typechecked under the assumptions
that $\mathit{x}$ and $\mathit{y}$ are bound to an injected value with $\ell$ and a
variant value discarding the first $\ell$ field, respectively.  Type-and-row
equivalence is extended with variant types naturally.


\subsection{Variants, gradually typed}

\begin{figure}[t]
 % type system
 \begin{flushleft}
  \input{defns/grad_lang/type_match}
  %
  \textbf{Typing and well-formedness rules} \quad
  \framebox{$\vdash  \Gamma$} \quad
  \framebox{$\Gamma  \vdash  \ottnt{A}  \ottsym{:}  \ottnt{K}$} \quad
  \framebox{$\Gamma  \vdash  \ottnt{M}  \ottsym{:}  \ottnt{A}$}
 \end{flushleft}
 \begin{center}
  \input{defns/grad_lang/typing_rules}
 \end{center}
 \caption{The extension of {\surfacelang} with variants.}
 \label{fig:variant:grad_lang}
\end{figure}

Once {\staticlang} is extended with variants, extending {\surfacelang} is easy.
The syntax is obtained by augmenting the one given by
\reffig{variant:static_lang} with the dynamic type.  Consistency and consistent
equivalence can be extended with variant types naturally since they are closed
under type constructors, and their equivalence in the form of
Theorem~\ref{thm:consistent-eq-consistent-equiv} still holds.  The type system
is extended with three new typing rules given in \reffig{variant:grad_lang}.
These rules are similar to the typing rules added by
\reffig{variant:static_lang} except for two points.  First, they use type
matching where variant types and row extensions are required.  Second, the types
$\ottnt{C}$ and $\ottnt{D}$ of the branches of a case expression do not have to be the
same but, instead, they have to be \emph{mergeable}.  The merging result
$\ottnt{C}  \oplus  \ottnt{D}$ is the type of the whole case expression.  We have many choices to
implement the merge operator $ \oplus $.  For example, $\ottnt{C}  \oplus  \ottnt{D}$ could be
defined to be $ \star $ for any $\ottnt{C}$ and $\ottnt{D}$ if we want gradual typing to
be close to dynamic typing.  Another possible choice is to define $\ottnt{C}  \oplus  \ottnt{D}$
to be $\ottnt{C}$ (or $\ottnt{D}$) if and only if $\ottnt{C}  \equiv  \ottnt{D}$; if $\ottnt{C}$ and $\ottnt{D}$
are not equivalent, $\ottnt{C}  \oplus  \ottnt{D}$ is undefined.  Such a definition might be
desirable for gradual typing to be strict as static typing.  We could also give
a compromising definition as in \citet{Garcia/Clark/Tanter_2016_POPL}.  In this
paper, instead of giving a concrete definition of $ \oplus $, we investigate
requirements to $ \oplus $ needed to prove properties of {\surfacelang}.  For
example, we require $\ottnt{C}  \oplus  \ottnt{D}$ to be consistent with both $\ottnt{C}$ and $\ottnt{D}$
in order to prove type preservation of translation from {\surfacelang} to
{\interlang}.  We discuss the other requirements in \sect{prop}.

\subsection{Variants, blamed}

\begin{figure}[t]
 % syntax
 \[\begin{array}{lrl}
  \syntaxGty{} \\[.5ex]
  \syntaxEterm{} \\[.5ex]
  \syntaxVvalue{} \\[.5ex]
  \syntaxEctx{}
 \end{array}\]
 %
 % semantics
 \begin{flushleft}
  \input{defns/blame/red_variant}
 \end{flushleft}
 %
 \caption{The extension of {\interlang} with variants.}
 \label{fig:variant:blame}
\end{figure}

Finally, we give an extension of {\interlang} with variants in
\reffig{variant:blame}.  Convertibility and the type system can be extended
easily, so we omit them in this section.

\paragraph{Syntax}
%
Types are augmented with variant types and terms are with injections, embedding
terms, and case expressions.  Values are extended with applications of injection
and embedding to values, casts to the variant type $ \langle  \star  \rangle $, and
conversions concealing the row of a variant type.  It is notable that embedding
$ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{v} } $ is a value even if embedded value $\ottnt{v}$ is an injection
tagged with a label different from $\ell$, while in the extended {\staticlang}
labels held by an embedding term and its underlying injection has to be the same
in order for the embedding term to be a value.  This is due to the lack of a
subsumption rule for type-and-row equivalence in {\interlang}.  For example,
injection $\ell \, \ottnt{v}$ can be given type $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;    \ell'  \mathbin{:}  \ottnt{B}   ;   \cdot     \rangle $ but cannot
be given $ \langle    \ell'  \mathbin{:}  \ottnt{B}   ;    \ell  \mathbin{:}  \ottnt{A}   ;   \cdot     \rangle $ in {\interlang}.  To embed $\ell \, \ottnt{v}$
into $ \langle    \ell'  \mathbin{:}  \ottnt{B}   ;    \ell  \mathbin{:}  \ottnt{A}   ;   \cdot     \rangle $, we use embedding: embedding value
$ \variantlift{ \ell' }{ \ottnt{B} }{ \ottsym{(}  \ell \, \ottnt{v}  \ottsym{)} } $ can have type $ \langle    \ell'  \mathbin{:}  \ottnt{B}   ;    \ell  \mathbin{:}  \ottnt{A}   ;   \cdot     \rangle $.
Conversely, if the type of value $\ottnt{v}$ is a variant type $ \langle    \ell  \mathbin{:}  \ottnt{A}   ;  \rho   \rangle $,
then $\ottnt{v}$ is either an injection value $\ell \, \ottnt{v'}$ or an embedding value
$ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{v'} } $ for some $\ottnt{v'}$.  Thus, the embedding operation is not only
useful to make variant types amenable in the setting with row
polymorphism---this motivates \citet{Leijen_2005_TFP} to introduce the embedding
operation---but also crucial to make a type system for variant types
syntax-directed.

\paragraph{Semantics}
%
\reffig{variant:blame} shows only reduction rules for case expressions and casts
between variant types; conversions for variant types reduce in a similar way as
ones for record types given in \reffig{blame:red_record}.  Reduction rules for
case expressions are similar to those of {\staticlang}, but they suppose that
injections and embedding terms hold the same label as the pattern.  The first
four cast reduction rules (\R{VIdName}--\R{VBlame}) are similar to the
corresponding rules for record types (\reffig{blame:red_record}).
%
The rule \R{VRevInj} is applied if injection $\ell \, \ottnt{v}$ is cast to a variant type
$ \langle  \rho_{{\mathrm{2}}}  \rangle $ having a $\ell$ field.  Let $\ottnt{A}$ be the type of $\ottnt{v}$,
and $\rho_{{\mathrm{21}}}$ and $\rho_{{\mathrm{22}}}$ be sequences of fields that appear prior and
posterior to the first, leftmost $\ell$ field in $\rho_{{\mathrm{2}}}$, respectively.  The
injection $\ell \, \ottsym{(}  \ottnt{v}  \ottsym{:}  \ottnt{A} \,  \stackrel{ \ottnt{p} }{\Rightarrow}  \ottnt{B}   \ottsym{)}$ can be given type $ \langle    \ell  \mathbin{:}  \ottnt{B}   ;  \rho_{{\mathrm{22}}}   \rangle $.  In
order for $\ell \, \ottsym{(}  \ottnt{v}  \ottsym{:}  \ottnt{A} \,  \stackrel{ \ottnt{p} }{\Rightarrow}  \ottnt{B}   \ottsym{)}$ to have type $ \langle  \rho_{{\mathrm{2}}}  \rangle  =  \langle    \rho_{{\mathrm{21}}}  \odot  \ottsym{(}    \ell  \mathbin{:}  \ottnt{B}   ;   \cdot    \ottsym{)}  \odot  \rho_{{\mathrm{22}}}    \rangle $, the reduction result applies the embedding
operation to $\ell \, \ottsym{(}  \ottnt{v}  \ottsym{:}  \ottnt{A} \,  \stackrel{ \ottnt{p} }{\Rightarrow}  \ottnt{B}   \ottsym{)}$ with all fields in $\rho_{{\mathrm{21}}}$.  Such a
sequence of embedding applications, written $ \variantliftrow{ \rho_{{\mathrm{21}}} }{ \ottsym{(}  \ell \, \ottsym{(}  \ottnt{v}  \ottsym{:}  \ottnt{A} \,  \stackrel{ \ottnt{p} }{\Rightarrow}  \ottnt{B}   \ottsym{)}  \ottsym{)} } $, is
defined as follows.
%
\input{defns/blame/row_embedding}
\noindent
%
If the cast value is an embedding value $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{v} } $, the rule \R{VRevLift}
is applied.  The reduction result first casts $\ottnt{v}$ to $ \langle    \rho_{{\mathrm{21}}}  \odot  \rho_{{\mathrm{22}}}    \rangle $ and then inserts field $ \ell  \mathbin{:}  \ottnt{A} $ at an appropriate position of $\rho_{{\mathrm{21}}}  \odot  \rho_{{\mathrm{22}}}$ by using case matching and embedding, which is formalized as follows.
%
\input{defns/blame/variant_field_insert}
\noindent
%
If $\rho_{{\mathrm{2}}}$ includes no $\ell$ field, either \R{VConInj} or \R{VConLift} is
applied depending on whether a cast value is injection $\ell \, \ottnt{v}$ or embedding
value $ \variantlift{ \ell }{ \ottnt{A} }{ \ottnt{v} } $.  In the former case, the injection $\ell \, \ottnt{v}$ is
injected into the variant type $ \langle  \star  \rangle $ and then embedded into type
$ \langle  \rho_{{\mathrm{2}}}  \rangle $.  In the latter, first the embedded value $\ottnt{v}$ is cast to
$ \langle  \rho_{{\mathrm{2}}}  \rangle $ and field $ \ell  \mathbin{:}  \ottnt{A} $ is inserted.  Then, the result is cast to
$ \langle  \rho_{{\mathrm{2}}}  \rangle $.  The field insertion is necessary to preserve the stack of
applications of the embedding operation.

\paragraph{Examples of reduction}
\TS{TODO?}

